Typing weak MSOL properties

We consider lambda-Y-calculus as a non-interpreted functional programming language: the result of the execution of a program is its normal form that can be seen as the tree of calls to built-in operations. Weak monadic second-order logic (wMSOL) is well suited to express properties of such trees. We give a type system for ensuring that the result of the execution of a lambda-Y-program satisfies a given wMSOL property. In order to prove soundness and completeness of the system we construct a denotational semantics of lambda-Y-calculus that is capable of computing properties expressed in wMSOL.

==> conclusion.tex <==
We have shown how to construct a model for a given weak alternating
tree automaton so that the value of a term in the model determines if
the B\"ohm tree of the term is accepted by the automaton. Our
construction builds on ideas from~\cite{SalWalTLCA} but requires to
bring out the modular structure of the model. This structure is very
rich, as testified by Galois connections.  This structure
allows us to derive type systems for wMSOL properties following the
``domains in logical form'' approach.

The type systems are relatively streamlined: the novelty is the
stratification of types used to restrict applicability of the greatest
fixpoint rule. 
Kobayashi and Ong~\cite{kobayashi09:_type_system_equiv_to_modal} were
the first to approach higher-order verification of MSOL properies
through typing. 
In their type system derivations are graphs, or infinite trees, and their validity is
defined via some regular acceptance condition on infinite paths. 
Their type system handles only
closed terms of type $o$, and fixpoint are handled via the condition
on infinite paths.
Tsukada and Ong have recently proposed a higher-order analogue of this
system~\cite{TsuOng14}.
The typability is defined in a standard way as the existence of a finite
derivation.
The semantics of the fixpoint combinator is defined via some special
games.
The soundness and completeness proofs use a syntactic approach.
In our case, thanks to the restriction to wMSO, we can use standard
fixpoint rules to handle the fixpoint combinator, we also obtain a
model allowing us to prove soundness and completeness using quite
standard techniques.


Typing in our system is decidable, actually the height of the
derivation is bounded by the size of the term. Yet the width can be
large, that is unavoidable given that the typability is $n$-\EXPTIME\
hard for terms of order
$n$~\cite{kobayashi09:_compl_model_check_recur_schem}.
Due to
the correspondence of the typing with semantics, every term has a
``best'' type.


While the paper focuses on typing, our model construction can be also
used in other contexts. It  allows us to immediately deduce
reflection~\cite{Broadbent:2010:RSL:1906484.1906730} and transfer~\cite{SalWalTransfer}
theorems for wMSOL. Our techniques used to construct models and prove their
correctness rely on usual techniques of domain
theory~\cite{amadio98:_domain_lambd_calcul}, offering an alternative,
and arguably simpler,
point of view to techniques based on unrolling.


The idea behind the reflection construction is to transform a given
term so that at every moment of its evaluation every subterm ``knows'' its
meaning in the model. In~\cite{Broadbent:2010:RSL:1906484.1906730} this property is
formulated slightly differently and is proved using a detour to
higher-order pushdown automata. Recently Haddad~\cite{Haddad13} has given a direct
proof for all MSOL properties. The proof is based on some notion of
applicative structure that is less constrained than  a model of the $\lambda Y$-calculus.
One could apply his construction, or take the one
from~\cite{SalWalTLCA}.
%  where we  have constructed models for divergence
% checking. We have given there a construction of a reflective term
% that works for all finitary models of the $\lambda Y$-calculus, in particular
% for those presented in this paper.

The transfer theorem says that for a fixed finite vocabulary of terms, an
MSOL formula $\f$ can be effectively transformed into an MSOL formula
$\wh\f$ such that for every term $M$ of type $o$ over the fixed vocabulary: $M$
satisfies $\wh\f$ iff the B\"ohm tree of M satisfies $\f$. Since the MSOL
theory of a term, that is a finite graph, is decidable, the transfer
theorem implies decidability of MSOL theory of B\"ohm trees of $\lambda
Y$-terms. As shown in~\cite{SalWalTransfer} it gives also a
number of other results.

A transfer theorem for wMSOL can be deduced from our model
construction. For every wMSOL formula $\f$ we need to find a formula
$\wh\f$ as above. For this we transform $\f$ into a weak alternating automaton
$\Aa$, and construct a model $\Dd_\f$ based on $\Aa$. Thanks to the
restriction on the vocabulary, it is quite easy to write for every
element $d$ of the model $\Dd_\f$ a wMSOL formula $\a_d$ such that for
every term $M$ of type $o$ in the restricted vocabulary:
$M\sat\a_d$ iff $\sem{M}^{\Dd_\f}=d$. The formula $\wh\f$ is then just a
disjunction $\Lor_{d\in F}\a_d$, where $F$ is the set elements of
$\Dd_\f$ characterizing terms whose B\"ohm tree satisfies $\f$.



% As underlined in the introduction, our type system is essentially
% different from the sytem of Kobayashi and
% Ong~\cite{kobayashi09:_type_system_equiv_to_modal}. In the later
% the difference between the least and the greatest fixpoint is captured
% by the rules of the game defined on the top of the type system. Our
% system uses standard fixpoint rules modulo taking in the account
% the stratification present in the model. Since fixpoints in our model
% are neither greatest not least fixpoints, some modification of the
% standard rules is unavoidable. Duality offered by games in Kobayashi
% and Ong system has been recently used to improve the sate of the art
% in model-checking algorithms. We hope that our type system can
% contribute to this line of research.

The fixpoints in our models are non-extremal: they are neither the
least nor the greatest fixpoints. From \cite{SalWalTLCA} we
know that this is unavoidable. We are aware of very few works
considering such cases.  Our models are an instance of cartesian
closed categories with internal fixpoint operation as studied by Bloom
and Esik~\cite{bloom96:_fixed}. Our model satisfies not only Conway
identities but also a generalization of the \emph{commutative axioms}
of iteration theories~\cite{bloom93:_iterat_theor}. Thus it is
possible to give semantics to the infinitary $\lambda$-calculus in our
models.  It is an essential step towards obtaining an algebraic
framework for weak regular
languages~\cite{blumensath13:_rabin_tree_theor}.

% \textbf{Clipings:} While we are working in uninterpreted setting, if
% we are given finite abstract domain, then in wMSOL it is possible to
% calculate the abstract value of a variable at a point of the tree. So
% questions of the form $BT(M)\sat\a$ can express analyses using finite
% domains. More importandly wMSOL can express


% Most existing model-checking tools handle only TAC automata. This is
% due the simplicity of Kobayashi's typing system mentioned above.
% Kobayashi and Ong~\cite{kobayashi09:_type_system_equiv_to_modal} have proposed a type based approach to
% model-checking of all MSOL properties. It consists of two steps: (i) a
% typing system is used to construct judgments about terms without
% fixpoints, (ii) these judgments are used to construct a parity game
% that is solved to determine if a property holds or not. So the
% semantics of fixpoints is given by games. Very
% recently~\cite{ramsay_type_refinement}, a new very promising
% model-checking algorithm using this approach has been proposed. It
% deals with both TAC automata and their duals, and exploits the duality
% between two players in the parity game.  It is likely that this idea can
% be adapted to our models since in our case fixpoints and the duality
% are present directly in the model.



% model we propose is an instance of a model with non-extremal
% fixpoint. As the model proposed in~\cite{SalWalTLCA}, it induces a
% Cartesian Closed Category (ccc) with, as coined
% in~\cite{bloom96:_fixed}, an \emph{internal} fixed-point operation.
% While in~\cite{bloom96:_fixed} the equational theory of \emph{Conway
%   ccc's}, that is ccc's with an internal fixpoint satisfying the
% so-called Conway identities, we here obtain not only a Conway ccc, but
% our model satisfy a generalization of the \emph{commutative axioms} of
% iteration theories\cite{bloom93:_iterat_theor}.  This has the
% fortunate advantage of inducing a semantics to the infinitary
% $\lambda$-calculus. Nevertheless, the study of those Conway ccc's that
% satisfy the commutative axioms remain to be done.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "m"
%%% End:

%  LocalWords:  wMSOL subterm Haddad MSOL applicative finitary iff Esik
%  LocalWords:  decidability fixpoints extremal fixpoint infinitary
%  LocalWords:  typability disjunction cartesian Kobayashi Ong


==> introduction.tex <==
Higher-order functional programs are more and more frequently used to write
interactive applications. In this context it is important to reason about
behavioral properties of programs.  We present a kind of type and
effect discipline~\cite{NN99}
%Mart ́ın Abadi, Andrew Birrell, Tim Harris, and Michael Isard. Se- mantics of transactional memory and automatic mutual exclu- sion. In POPL ’08: Proceedings of the 35th Annual ACM
%John M. Lucassen and David K. Gi↵ord. Polymorphic e↵ect systems. In Jeanne
%Ferrante and P. Mager, editors, POPL, pages 47–57. ACM Press, 1988.
%RobertGrabowskietal.Type-basedenforcementofsecureprogrammingguidelines
%- code injection prevention at sap. FAST, LNCS 7140, pp
%182–197. Springer, 2011.
where a well-typed program will satisfy behavioral properties
expressed in weak monadic second-order logic (wMSOL).

We consider the class of programs written in the simply-typed calculus
with recursion and finite base types: the $\lambda Y$-calculus.  This calculus
offers an abstraction of higher-order programs that faithfully
represents higher-order control. The dynamics of an interaction of a
program with its environment is represented by the B\"ohm tree of a
$\lambda Y$-term that is a tree reflecting the control flow of the
program. For example, the B\"ohm tree of the term $Y x. ax$ is the
infinite sequence of $a$'s, representing that the program does an
infinite sequence of $a$ actions without ever terminating.
Another example is presented in Figure~\ref{fig:fact}. A functional
program for the factorial function is written as a $\lambda Y$-term
$\Fct$ and the value of $\Fct$ applied to a constant $c$ is calculated.
Observe that all constants in $\Fct$ are non-interpreted.
The B\"ohm tree semantics reflects the call-by-name
evaluation strategy. Nevertheless, the call-by-value evaluation can be encoded, so
can be finite data domains and conditionals over
them~\cite{hillebrand94:_finit_model_theor_in_simpl,KobACM,Haddad13}. The approach
is then to translate a functional program to a $\lambda Y$-term and to
examine the B\"ohm tree it generates.
\begin{figure}[tbh]
\includegraphics[scale=.35]{factorial.pdf}
%   \centering
%   \newcommand{\ifte}{\textbf{if}}
% \begin{tikzpicture}
% \draw (0,2) node{$Factorial(x)\ \equiv\ \mathbf{if}\ x=0\ \mathbf{then}\ 1\
%       \mathbf{else}\ x\cdot Factorial(x-1) $};
%     \draw (0,1) node{$\Fct\ \equiv\  Y F.\ \lambda x.\ \mathbf{if}\ %
%       (z\ x)\ 1\ (m\ x\ (\Fct (-\ x\ 1))))$};
% \draw (-3,0) node{$BT(\Fct\ c)$ is};
%  \node {\ifte}[grow=down,level distance=3.5ex]
%   child {node {$z$}
%     child {node {$c$}}}
%   child {node {$1$}}
%   child {node {$m$}
%     child {node {$c$}}
%     child {node{\ifte}
%       child {node {$z$}
%     child {node{$-$}
%       child {node{$c$}}
%       child {node {$1$}}}}
%   child {node {$1$}}
%   child {node {$m$}
%     child {node {\vdots}}}
% }};
% \end{tikzpicture}
  \caption{B\"ohm tree of the factorial function}
  \label{fig:fact}
\end{figure}


Since the dynamics of the program is represented by a potentially
infinite tree, monadic second-order logic (MSOL) is a natural
candidate for the language to formulate properties in. This logic is
an extension of first-order logic with quantification over sets.  MSOL
captures precisely regular properties of trees~\cite{rabin69}, and it is
decidable if the B\"ohm tree generated by a given $\lambda Y$-term
satisfies a given property~\cite{Ong06}. In this paper we will restrict
to weak monadic second-order logic (wMSOL). The difference is that in
wMSOL quantification is restricted to range over finite sets.  While
wMSOL is a proper fragment of MSOL, it is sufficiently strong to express
safety, reachability, and many liveness properties. Over sequences, that is,
degenerated trees where every node has one successor, wMSOL is
equivalent to full MSOL.

The basic judgments we are interested in are of the form $BT(M)\sat\a$
meaning that the result of the evaluation of $M$, i.e.\ the B\"ohm
tree of $M$, has the property $\a$ formulated in wMSOL. Going back to
the example of the factorial function from Figure~\ref{fig:fact}, we
can consider a property: all computations that eventually take the
middle branch in a node labeled by ``if'' are finite. This property
holds in
$BT(\Fct\ c)$. Observe by the way that $BT(\Fct\
c)$ is not regular -- it has infinitely many non-isomorphic subtrees
as the number of subtractions occurring in the left branches of ``if''
nodes is growing with the depth of those nodes. In general, the interest of
judgments of the form $BT(M)\sat\a$ is due to their ability to express liveness
and fairness properties of executions, like: ``every \emph{open}
action is eventually followed by a \emph{close} action'', or that
``there are infinitely many read actions''.  Various other
verification problems for functional programs can be reduced to this
problem~\cite{KobACM,KobTabUnn10,OngRam11,TobitaTK12,GrabowskiHL11}.
% \begin{figure}[tbh]
%   \centering
%   \includegraphics[scale=.42]{property.pdf}
%   \caption{A wMSOL property of a B\"ohm tree. A possible valuation of
%     quantified variables $x$ and $Z$ is highlighted.}
%   \label{fig:formula}
% \end{figure}

Technically, the judgment $BT(M)\sat\a$ is equivalent to determining
whether a B\"ohm tree of a given $\lambda Y$-term is accepted by a given
weak alternating automaton. This problem is known to be decidable
thanks to the result of Ong~\cite{Ong06}, but we hope that the denotational
approach we are pursuing here brings additional benefits. Our two main
contributions are:
\begin{itemize}
\item A construction of a finitary model for a given weak
  alternating automaton. 
  The ranking condition on the automaton is lifted to the denotational
  model and reflected in the alternation of the least and greatest
  fixpoints. 
  The value of a term in this model determines
  if the B\"ohm tree of the term is accepted by the automaton. So
  verification is reduced to evaluation in the model.
\item Two type systems. A typing system deriving statements of the
  form ``the value of a term $M$ is bigger than an element $d$ of the
  model''; and a typing system for dual properties. These typing
  systems use standard fixpoint rules and  follow the methodology
  coined as \emph{Domains in Logical Form}
  \cite{abramsky91:_domain_theor_logic_form}. Thanks to the first
  item, these typing systems can directly talk about
  acceptance/rejection of the B\"ohm tree of a term by an
  automaton. These type systems are decidable, and every term has a
  ``best'' type that simply represents its value in the model.
\end{itemize}

Having a model and a type system has several advantages over having
just a decision procedure. First, it makes verification compositional:
the result for a term is calculated from the results for its subterms.
In particular, it opens possibilities for a modular approach to the
verification of large programs.  Next, it enables semantic based
program transformations as for example reflection of a given property
in a given
term~\cite{Broadbent:2010:RSL:1906484.1906730,SalWalTLCA,Haddad13}. It
also implies the transfer theorem for wMSOL~\cite{SalWalTransfer} with
a number of consequences offered by this theorem.  Finally, models
open a way to novel verification algorithms be it through evaluation,
type system, or through hybrid algorithms using typing and evaluation
at the same time~\cite{terui_semantic_evaluation}. We come back to
these points in the conclusions.
\medskip

\emph{Related work.} Historically, Ong~\cite{Ong06} has shown the
decidability of the MSOL theory of B\"ohm trees for all $\lambda Y$-terms.
This result has been revisited in several different ways. Some
approaches take a term of the base type, and unroll it to some
infinite object: tree with pointers~\cite{Ong06}, computation of a
higher-order pushdown automaton with
collapse~\cite{Hague08:collapsible_pushdown_automata_and_recursion_schemes},
a collection of typing judgments that are used to define a
game~\cite{kobayashi09:_type_system_equiv_to_modal}, a computation of
a Krivine machine~\cite{SalWalKrivine_machine}. Recently, Tsukada
and Ong~\cite{TsuOng14} have presented a compositional approach: they
give a typing system where the notion of a derivation is standard,
their types are extended with annotations, and 
the fixpoint combinator is defined via game on these types with
annotations.  We will comment more on the relation with this work
after we introduce our type system, as well as in the conclusions. 
Another recent advance is given by Hofmann
and Chen~\cite{CheHof14} who provide a type system for verifying path
properties of trees generated by first-order $\lambda Y$-terms.  In
other words, this last result gives a typing system for verifying path
properties of trees generated by deterministic pushdown
automata. Compared to this last work, we consider the whole
$\lambda Y$-calculus and an incomparable set of properties.

Already some time ago, Aehlig~\cite{aehlig07} has discovered an easy
way to prove Ong's theorem restricted to properties expressed by tree
automata with trivial acceptance conditions (TAC automata).  The core
of his approach can be formulated by saying that the verification
problem for such properties can be reduced to evaluation in a
specially constructed and simple model.  Later, Kobayashi proposed a
type system for such properties and constructed a tool based on
it~\cite{KobACM}. This in turn opened a way to an active ongoing
research resulting in the steady improvement of the capacities of the
verification
tools~\cite{Kob09,BroadbentCHS13,BroadbentK13,RamsayNO14}.  TAC
automata can express only safety properties.  Our models consist of
layers of models used by Aehlig, and our type system is a layered
version of Kobayashi's system.  
This close relation to the model and type system for trivial
properties, makes us hope that our model and
typing system can be useful for practical verification of wMSOL
properties. 
% Indeed the organization of the model and of the type
% system can be seen as a natural extension of the ones dealing with
% trivial properties. It should thus be not to difficult to extend the
% algorithmic methods already developed by the community for trivial
% properties so as to obtain efficient verification algorithm for wMSOL
% properties.

The model approach to verification of $\lambda Y$-calculus is quite
recent. In~\cite{SalWalTLCA} it is shown that simple models with
greatest fixpoints capture exactly properties expressed with TAC
automata. An extension is then proposed to allow one to detect
divergence. The simplicity offered by models is exemplified by
Haddad's recent work~\cite{Haddad13} giving simple
semantic based transformations of $\lambda Y$-terms.


We would also like to mention two other quite different approaches to
integrate properties of infinite behaviors into typing. Naik and
Palsberg~\cite{NaikP08} make a connection between model-checking and
typing. They consider only safety properties, and since their setting
is much more general than ours, their type system is more
complex too. Jeffrey~\cite{Jef12,Jef14} has shown how to incorporate
Linear Temporal Logic into types using a much richer dependent types
paradigm. The calculus is intended to talk about control and data in
functional reactive programming framework, and aims at using SMT
solvers.  \medskip
 % Finally the construction of a
% model requires, at the level of infinite objects, to find the right
% abstraction that captures the targeted properties.  Examples of such
% advances are given by Wilke
% algebras~\cite{wilke91:_eilen_theor_infin_languag} for infinite words
% of by the recent notion of $\w$-hyperclones by
% Blumensath~\cite{blumensath13:_rabin_tree_theor}.  Moreover, such a
% construction also requires to tie the abstraction with the evaluation
% of $\lambda$-calculus so that the properties can be verified in the flow of
% a higher-order program.  Therefore such constructions involve a
% delicate integration of algebraic methods with denotational semantics
% and shed light on the nature of the captured set of properties.




\emph{Organization of the paper.} In the next section we introduce
the main objects of our study: $\lambda Y$-calculus, and weak
alternating automata.  Section~\ref{sec:type-system} presents the type
system. Its soundness and completeness can be straightforwardly
formulated for closed terms of atomic type. For the proof though, we
need a statement about all terms. This is where the model based
approach helps.  Section~\ref{sec:model-wmso} describes how to
construct models for wMSOL properties.
% We then show in
% Section~\ref{sec:corr-compl-model} that our models
% indeed capture weak alternating automata
% (Theorem~\ref{thm:model-correct}).
In Section~\ref{sec:from-model-type} we come back to our type systems.
The general soundness
and completeness property we prove says that types can denote every element
of the model, and the type systems can derive precisely the
judgments that hold in the model
(Theorem~\ref{thm:types_correctness_completeness}).  In the conclusion
section we mention other applications of our model.
%All proofs can be
%found in a long version of the paper~\cite{salvati:hal-01061202}.

% Interestingly, the model we propose for wMSOL, preserves the duality
% present in the model for trivial properties.  This duality has been
% recently exploited to propose the presently most efficient algorithm
% for model checking higher-order schemes trivial properties~\cite{}.
% We here show how to exploit this duality by proposing two dual type
% systems that capture valuations in the models. One allows to checks
% whether the B\"ohm tree of a term is accepted in a given state while
% the other shows that there is no accepting run from a given state.


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "m"
%%% End:

%  LocalWords:  wMSOL BT MSOL reachability liveness subtrees Ong Schupp
%  LocalWords:  denotational finitary fixpoint compositional subterms
%  LocalWords:  Knapik Niwinski Urzyczyn decidability Krivine Tsukada
%  LocalWords:  Hofmann Aeligh Ong's TAC Kobayashi fixpoints Haddad's
%  LocalWords:  Naik Palsberg SMT


==> preliminaries.tex <==
We quickly fix notations related to the simply typed $\lambda Y$-calculus
and to B\"ohm trees.  We then recall the definition of weak
alternating automata on ranked trees. These will be used to specify
properties of B\"ohm trees.  Finally, we introduce the notion of the
greatest fixpoint models for the $\lambda Y$-calculus. This notion allows
us to adapt the definition of recognizability from language theory, so
models can be used to define sets of terms. These sets of terms are
closed under the reduction rules of the $\lambda Y$-calculus. We recall the
characterization, in terms of automata, of the sets of terms
recognizable by the greatest fixpoint models.  \medskip


The \emph{set $\Tt$ of types  of $\lambda Y$-calculus}  is constructed from a unique \emph{basic
  type} $o$ using a binary operation $\to$ that associates to the
right\footnote{We use a unique atomic type, but our approach generalizes
without problems to any number of atomic types.}. Thus $o$ is a type and if
$A$, $B$ are types, so is $(A\to B)$. The order of a type is defined
by: $\order(o)=0$, and $\order(A\to B)=max(1+\order(A),\order(B))$.
We work with \emph{tree signatures} that are finite sets of
\emph{typed constants of order at most $1$}.  % Typed constants are symbols
% associated with types of order $1$.
Types of order $1$ are of the form $o\to\dots\to o\to o$ that we
abbreviate $o^i\to o$ when they contain $i+1$ occurrences of $o$. For convenience we assume that $o^0\to o$ is
just $o$. If $\S$ is a signature, we write $\S^{(i)}$ for the set of constants of
type $o^i\to o$.
In examples we will often use constants of type
$o\to o$ as this makes the examples more succinct.
At certain times, we will restrict to the types $o$ and
$o^2\to o$ that are representative for all the cases.
\medskip

\looseness=-1
\emph{Simply typed $\lambda Y$-terms} are built from the
constants in the signature, and constants $Y^{A}$, $\W^A$ for every
type $A$. These stand for the \emph{fixpoint combinator} and
\emph{undefined term}, respectively. The fixpoint combinators
allows to have have computations with a recursion. 
The undefined terms represent
diverging computation, but also, at a technical level are used to
construct finite approximations of infinite computations.
Apart from constants, for each
type $A$ there is a countable set of variables $x^A,y^A,\dots$. Terms
are built from these constants and variables using typed application:
if $M$ has type $A\to B$ and $N$ has type $A$, then $(MN)$ has type
$B$;
and $\lambda$-abstraction: if $M$ has type $B$ then $(\lambda x^A. M)$ has type
$A\to B$. We shall remove unnecessary parentheses, in particular, we
write sequences of applications $((N_0 N_1) \dots N_ n) $ as $N_0
\dots N_n$ and we write sequences of $\lambda$-abstractions
$\lambda x_1.\dots \lambda x_n.\ M$ with only one $\lambda$: either $\lambda x_1\dots
x_n.\ M$, or even shorter $\lambda \vec x.\ M$. We will often write $Y x.M$
instead of $Y(\lambda x.M)$. Every $\lambda Y$-term can be written in this
notation since $YN$ has the same B\"ohm tree as $Y(\lambda x. N x)$,
and the latter term is $Yx. (Nx)$\label{notation:Yx}. We write
$M[x_1:=N_1,\dots,x_n:=N_n]$ for the term obtained from $M$ by the
simultaneous capture-avoiding substitution of $N_1$, \dots, $N_n$ for
the variables $x_1$, \dots, $x_n$. All the substitutions we shall
consider map variables to terms of the same type. When working with an
abstract substitution $\s$, we write $M.\s$ for the term obtained by
applying $\s$ to $M$. We use the usual operational semantics of
the calculus, $\beta\delta$-reduction ($\stackrel{\ast}{\to}_{\beta\delta}$)
which is the reflexive transitive closure of the union of the
relations of $\beta$-contraction ($\to_\beta$) and $\delta$-contraction
($\to_\delta$) which are the following rewriting relations:
$$(\lambda x.M)N \to_\beta M[x:=N] \quad Y M \to_\delta M(Y M)$$

% We take for
% granted the operational semantics of the calculus given by $\beta$ and
% $\delta$ reductions. We also take for granted the notion of
% capture-avoiding substitution and given a substitution $\s$ and a term
% $M$, we write $M.\s$ to denote the term obtained from $M$ after
% applying the substitution $\s$.
% The usual operational semantics of the $\lambda$-calculus is given by
% $\beta$-contraction. To give the meaning to fixpoint constants we use
% $\delta$-contraction ($\to_\delta$):
% $(\lambda x. M)N\to_\beta M[N/x]$ and  $YM\to_\delta M (YM)$.
% A \emph{B\"ohm tree} is an unranked, ordered, and potentially infinite
% tree with nodes labeled by terms of the form $\lambda x_1.\dots x_n. N$;
% where $N$ is a variable or a constant, and the sequence of
% $\lambda$-abstractions is optional. So for example $x^0$, $\W^0$, $\lambda
% x^0. \W^0$ are labels, but $\lambda y^0.\ x^{0\to 0} y^0$ is not.
\begin{defi}
  The \emph{B\"ohm tree} of a term $M$ is a possibly infinite labeled
  tree that is defined co-inductively.  If $M$ can be reduced so as to
  obtain a term of the form $\lambda \vec x.N_0N_1\dots N_k$ with $N_0$ a
  variable or a constant, then $BT(M)$ is a tree whose root is labeled
  by $\lambda \vec x.N_0$ and the immediate successors of its root are
  $BT(N_1)$, \dots, $BT(N_k)$. Otherwise $BT(M)$ is a single node tree
  whose root is labeled $\W^A$, where $A$ is the type of $M$.
\end{defi}
B\"ohm trees are infinite normal forms of $\lambda Y$-terms. A B\"ohm tree
of a closed term of type $o$ over a tree signature is a potentially
infinite ranked tree: a node labeled by a constant $a$ of type $o^i\to
o$ has $i$ successors (c.f.\ Figure~\ref{fig:fact}).

\paragraph{\bf Example}\label{ex:one}
% As a simple example, let us take $M= \lambda x. ax$. We have a
% reduction sequence
% $$YM\to_{\delta} (\lambda x. a x)(YM)\to_\beta a(YM)\cdots\to_{\beta\delta}
% a(a(YM))\to\dots$$
%  So $BT(YM)$ is the infinite sequence $aa\dots$

%  For a more complicated
As an example take $(YF.\ N) a$
 where $N=\lambda g.g(b(F(\lambda x. g(g\, x))))$. Both $a$ and $b$ have the
 type $o\to o$; while $F$ has type $(o\to o)\to o$, and so does $N$.
 Observe that we are using a more convenient notation $YF$ here.
 The B\"ohm tree of $(Y F. N)a$ is
 $BT((Y F.N)a) = ab a^2 b a^4 b\dots a^{2^n}b \dots$
after every consecutive occurrence of $b$ the number of occurrences of
$a$ doubles because of the double application of $g$ inside $N$.


\paragraph{\bf wMSOL and weak alternating automata}
We will be interested in properties of trees expressed in weak monadic
second-order logic. This is an extension of first-order logic with
quantification over finite sets of elements. The interplay of negation
and quantification allows the logic to express many infinitary
properties. The logic is closed for example under constructs: ``for
infinitely many vertices a given property holds'', ``every path consisting of
vertices having a given property is finite''. From the automata
point of view, the expressive power of the logic is captured by weak
alternating automata.

A \emph{weak alternating automaton} works on trees over a fixed tree
signature~$\S$. It is a tuple:
\begin{equation*}
  \Aa=\struct{Q,\S,q^0\in Q,\set{\delta_i}_{i\in\Nat},\rho:Q\to\Nat}
\end{equation*}
where $Q$ is a finite set of states, $q^0\in Q$ is the initial state,
$\rho$ is the \emph{rank function}, and $\delta_i:Q\times \S^{(i)} \to
\Pp(\Pp(Q)^i)$ is the transition function.  For $q$ in $Q$, we call
$\rho(q)$ \emph{its rank}.  The automaton is \emph{weak} in the sense
that when $(S_1,\dots,S_i)$ is in $\delta_i(q,a)$, then the rank of every
$q'$ in $\bigcup_{1\leq j\leq i} S_j$ is not bigger than the rank of
$q$, i.e. $\rho(q')\leq \rho(q)$.

Observe that since $\S$ is finite, only finitely many $\delta_i$ are
non-empty functions.
From the definition it follows that $\delta_2: Q\times \S^{(2)} \to
\Pp(\Pp(Q)\times\Pp(Q))$ and
$\delta_0:Q\times\S^{(0)}\to\set{\es,\set{()}}$. 
We will simply write $\delta$ without a subscript when this causes no ambiguity.
%The weakness requirement means that in the run the ranks cannot increase.


Automata will work on $\S$-labeled  trees that are partial
functions $t:\Nat^*\stackrel{\cdot}{\to}\S\cup\set{\W}$ whose domain
of definition satisfies the usual requirements, and such that the
number successors of a node is determined by the label of the node. In
particular, if $t(u) \in \S^{(0)}\cup\set{\W}$ then $u$ is a leaf.

\looseness=-1
\label{df:acceptance-game}The acceptance of a tree is defined in
terms of \emph{games} between two players that we call Eve and Adam.  A
\emph{play} between Eve and Adam from some node $v$ of a tree $t$ and
some state $q\in Q$ proceeds as follows.  If $v$ is a leaf and is
labeled by some $c\in \S^{(0)}$ then Eve wins iff $\delta_0(q,c)$ holds
(i.e. $\delta_0(q,c)$ is not empty). If
$v$ is labeled by $\W$ then Eve wins iff the rank of $q$ is
even.  Otherwise, $v$ is an internal node: Eve
chooses a tuple of sets of states $(S_1,\dots,S_i)\in\delta(q,t(v))$; then Adam
chooses $S_j$ (for $j=1,\dots,i$) and a state $q'\in S_j$. The play
continues from the $j$-th son of $v$ and state $q'$.
When a player is not able to play any move, he/she looses.
If the play is
infinite then the winner is decided by looking at ranks of states
appearing on the play.  Due to the weakness of $\Aa$, the rank of
states in a play can never increase, so it eventually stabilizes at
some value. Eve wins if this value is even. A tree $t$ is
\emph{accepted} by $\Aa$ from a state $q\in Q$ if Eve has a winning
strategy in the game started from the root of $t$ and from $q$.

Automata with \emph{trivial acceptance conditions}, as considered by
Kobayashi~\cite{Kob09}, are obtained by requiring that all states have
rank $0$. Automata with co-trivial conditions are just the ones where
all states have rank $1$.

Observe that without a loss of generality we can assume that $\delta$ is
monotone, i.e. if $(S_1,\dots,S_i)\in\delta(q,a)$ then for every
$(S'_1,\dots,S'_i)$ such that $S_j\incl S'_j\incl \set{q' : \rho(q')\leq
  \rho(q)}$ we have $(S'_1,\dots,S'_i)\in\delta(q,a)$. Indeed, adding the
transitions needed to satisfy the monotonicity condition does not give
Eve more winning possibilities.

An automaton defines a language of closed terms of type $o$, it
consists of terms whose B\"ohm
trees are accepted by the automaton from its initial state $q^0$:
$$L(\Aa)=\set{M\,:\, \text{$M$ is closed term of type $o$, $BT(M)$
 is accepted by $\Aa$ from $q^0$}}\ .$$

Observe that $L(\Aa)$ is closed under $\beta\delta$-conversion since the
Church-Rosser property of the calculus implies that two
$\beta\delta$-convertible terms have the same B\"ohm tree.

\paragraph{\bf Example}\label{ex:automaton} Consider a weak alternating automaton $\Aa$
defining the property ``action $b$ appears infinitely often''. The
automaton has
states $Q=\set{q_1,q_2}$, and the signature $\S=\set{a,b}$ consisting
of two constants of type $o\to o$. Over this signature, the B\"ohm trees are
just sequences. The transitions of $\Aa$ are:
\begin{align*}
  \delta(q_1, a) &= \set{q_1} &  \delta(q_2, a) &= \set{q_1,q_2}\\
  \delta(q_1, b) &  =\es &
  \delta(q_2, b) &= \set{q_2}
\end{align*}
The ranks of states are indicated by their subscripts. When started in $q_2$
the automaton spawns a run from $q_1$ each time it sees letter $a$. The
spawned runs must stop in order to accept, and they stop when they see
letter $b$ (cf. Figure~\ref{fig:run}). So every $a$ must be eventually
followed by $b$.
\begin{figure}[tbh]
  \centering
  \includegraphics[scale=.4]{alt-run.pdf}
  \caption{A run of an alternating automaton on $a\dots ab\dots$}
  \label{fig:run}
\end{figure}


\paragraph{\bf Models.}
We use standard notions and notations for models for $\lambda Y$-calculus,
in particular for \emph{valuation/variable assignment} and of
\emph{interpretation of a term}
(see~\cite{hindley08:_lambd_calcul_combin}). We shall write
$\sem{M}^\Ss_\nu$ for the interpretation of a term $M$ in a model
$\Ss$ with the valuation $\nu$.  As usual, we will omit subscripts or
superscripts in the notation of the semantic function if they are
clear from the context.

The simplest models of $\lambda Y$-calculus are based on monotone
functions.  A \emph{GFP-model} of a signature $\S$ is a tuple
$\Ss=\struct{\set{\Ss_A}_{A\in\Tt},\rho}$ where $\Ss_o$ is a finite
lattice, called the \emph{base set} of the model, and for every type
$A\to B\in \Tt$, $\Ss_{A\to B}$ is the lattice $\monf{\Ss_A}{\Ss_B}$
of monotone functions from $\Ss_A$ to $\Ss_B$ ordered
coordinate-wise. The valuation function $\rho$ is required to interpret
$\W^A$ as the greatest element of $\Ss_A$, and $Y^{A}$ as
the greatest fixpoint operator of functions in $\Ss_{A\to A}$. Observe that
every $\Ss_A$ is
finite, hence all the greatest fixpoints exist without any additional
assumptions on the lattice.



% A \emph{variable assignment} is a function $\val$ associating to a
% variable of type $A$ an element of $\Ss_A$. If $s$ is an element of
% $\Ss_A$ and $x^A$ is a variable of type $A$ then $\val[s/x^A]$ denotes
% the valuation that assigns $s$ to $x^A$ and that is identical to $\val$
% otherwise.

% The \emph{interpretation of a term} $M$ of type $A$ in the model
% $\Ss$ under the valuation $\val$ is an element of $\Ss_A$ denoted
% $\sem{M}_\Ss^\val$. The meaning is defined inductively:
% \begin{itemize}
% \item $\sem{c}^\val_\Ss=\rho(c)$
% \item $\sem{x^A}^\val_\Ss=\val(x^A)$
% \item
%   $\sem{MN}^\val_\Ss=\sem{M}^\val_\Ss(\sem{N}^\val_\Ss)$
% \item $\sem{\lambda x^A.M}^\val_\Ss$ is a function mapping an element
%   $s\in \Ss_A$ to $\sem{M}^{\val[s/x^A]}_\Ss$ that by abuse of
%   notation we may write $\lambda s.\sem{M}^{\val[s/x^A]}_\Ss$.
% \end{itemize}
% As usual, we will omit subscripts or superscripts in the notation of
% the semantic function if they are clear from the context.

We can now adapt the definition of recognizability by semigroups taken
from language theory to our richer models.
\begin{defi}\label{df:recognizability}
A GFP model $\Ss$ over the
base set $\Ss_o$ \emph{recognizes a language} $L$ of closed $\lambda
Y$-terms of type $o$ if
there is a subset $F\incl \Ss_o$ such that $L=\set{M \mid
  \sem{M}^\Ss\in F}$.
\end{defi}
%% The existence of a syntactic model is true for simply type
%% lambda-calculus
%% For the lambda Y-calculus we need terms to take the same value in
%% every finite monotone models to get the equality of their Bohm trees.
A direct consequence of Statman's finite completeness
theorem~\cite{Statman82} is that such models can characterize a term
up to equality:
$BT(M)=BT(N)$ iff the values of $M$ and $N$ are the
same in every monotone models. This property is sufficient for our
purposes. The celebrated result of Loader~\cite{Loader01} implies that
we cannot hope for a much stronger completeness property, and have good
algorithmic qualities at the same time.

The following theorem characterizes the recognizing power of GFP
models.
\begin{thm}[\cite{SalWalTLCA}]\label{thm:GFP-model}
  A language $L$ of $\lambda Y$-terms is recognized by a GFP-model iff
  it is a boolean combination of languages recognized by weak
  automata whose all states have rank $0$.
\end{thm}

% For the unfamiliar reader  a small
% example is presented in the appendix.
%Observe that $L(\Aa)$ is closed under $\beta\delta$-conversion.%  since the
% Church-Roser property of the calculus implies that two
% $\beta\delta$-convertible terms have the same B\"ohm tree.

% \paragraph{Example}\label{ex:automaton} Consider a weak alternating automaton $\Aa$
% defining the property ``action $b$ appears infinitely often''. The
% automaton has
% states $Q=\set{q_1,q_2}$, and the signature $\S=\set{a,b}$ consisting
% of two constants of type $o\to o$. Over this signature, the B\"ohm trees are
% just sequences. The transitions of $\Aa$ are:
%   $$\delta(q_1, a)=\set{q_1} \quad  \delta(q_2, a) = \set{q_1,q_2}
%   \delta(q_1, b)   =\es \quad
%   \delta(q_2, b) = q_2$$
% The ranks of states are indicated by their subscripts. When started in $q_2$
% the automaton spawns a run from $q_1$ each time it sees letter $a$. The
% spawned runs must stop in order to accept, and they stop when they see
% letter $b$.  %(cf. Figure~\ref{fig:run}).
% So every $a$ must be eventually
% followed by $b$.
% \begin{figure}[tbhf]
%   \centering
%   \includegraphics[scale=.35]{alt-run.pdf}
%   \caption{A run of an alternating automaton on $a\dots ab\dots$}
%   \label{fig:run}
% \end{figure}
%
% \medskip
%
% \subsection*{Models}
% We use standard notions and notations for models for $\lambda Y$-calculus,
% in particular for \emph{valuation/variable assignment} and of
% \emph{interpretation of a term}
% (see~\cite{hindley08:_lambd_calcul_combin}). We shall write
% $\sem{M}^\Ss_\nu$ for the interpretation of a term $M$ in a model
% $\Ss$ with the valuation $\nu$.  As usual, we will omit subscripts or
% superscripts in the notation of the semantic function if they are
% clear from the context.

% The simplest models of $\lambda Y$-calculus are based on monotone
% functions.  A \emph{GFP-model} of a signature $\S$ is a tuple
% $\Ss=\struct{\set{\Ss_A}_{A\in\Tt},\rho}$ where $\Ss_o$ is a finite
% lattice, called the \emph{base set} of the model, and for every type
% $A\to B\in \Tt$, $\Ss_{A\to B}$ is the lattice $\monf{\Ss_A}{\Ss_B}$
% of monotone functions from $\Ss_A$ to $\Ss_B$ ordered
% coordinate-wise. The valuation function $\rho$ is required to interpret
% $\W^A$ as the greatest element of $\Ss_A$, and $Y^{A}$ as
% the greatest fixpoint of functions in $\Ss_{A\to A}$. Observe that
% every $\Ss_A$ is
% finite, hence all the greatest fixpoints exist without any additional
% assumptions on the lattice.



% % A \emph{variable assignment} is a function $\val$ associating to a
% % variable of type $A$ an element of $\Ss_A$. If $s$ is an element of
% % $\Ss_A$ and $x^A$ is a variable of type $A$ then $\val[s/x^A]$ denotes
% % the valuation that assigns $s$ to $x^A$ and that is identical to $\val$
% % otherwise.

% % The \emph{interpretation of a term} $M$ of type $A$ in the model
% % $\Ss$ under the valuation $\val$ is an element of $\Ss_A$ denoted
% % $\sem{M}_\Ss^\val$. The meaning is defined inductively:
% % \begin{itemize}
% % \item $\sem{c}^\val_\Ss=\rho(c)$
% % \item $\sem{x^A}^\val_\Ss=\val(x^A)$
% % \item
% %   $\sem{MN}^\val_\Ss=\sem{M}^\val_\Ss(\sem{N}^\val_\Ss)$
% % \item $\sem{\lambda x^A.M}^\val_\Ss$ is a function mapping an element
% %   $s\in \Ss_A$ to $\sem{M}^{\val[s/x^A]}_\Ss$ that by abuse of
% %   notation we may write $\lambda s.\sem{M}^{\val[s/x^A]}_\Ss$.
% % \end{itemize}
% % As usual, we will omit subscripts or superscripts in the notation of
% % the semantic function if they are clear from the context.

% We can now adapt the definition of recognizability by semigorups taken
% from language theory to our richer models.
% \begin{defi}\label{df:recognizability}
% A GFP model $\Ss$ over the
% base set $\Ss_o$ \emph{recognizes a language} $L$ of closed $\lambda
% Y$-terms of type $o$ if
% there is a subset $F\incl \Ss_o$ such that $L=\set{M \mid
%   \sem{M}^\Ss\in F}$.
% \end{defi}
% %% The existence of a syntactic model is true for simply type
% %% lambda-calculus
% %% For the lambda Y-calculus we need terms to take the same value in
% %% every finite monotone models to get the equality of their Bohm trees.
% An direct consequence of Statman's finite completeness
% theorem~\cite{Statman82} is that such models can characterize a term
% up to equality:
% $BT(M)=BT(N)$ iff the values of $M$ and $N$ are the
% same in every monotone models. This property is sufficient for our
% purposes. The celebrated result of Loader~\cite{Loader01} implies that
% we cannot hope for a much stronger completeness property, and have good
% algorithmic qualities at the same time.

% The following theorem characterizes the recognizing power of GFP
% models.
% \begin{thm}[\cite{SalWalTLCA}]\label{thm:GFP-model}
%   A language $L$ of $\lambda Y$-terms is recognized by a GFP-model iff
%   it is a boolean combination of languages recognized by weak
%   automata whose all states have rank $0$.
% \end{thm}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "m"
%%% End:

%  LocalWords:  fixpoint recognizability combinator YN Yx Nx BT YM aa
%  LocalWords:  subtrees YF wMSOL infinitary monotonicity Roser GFP
%  LocalWords:  fixpoints semigorups Statman's Kobayashi


==> type-system1.tex <==
In this section we describe the main result of the paper.  We present
a type system to reason about wMSOL properties of B\"ohm trees of
terms. We will rely on the equivalence of wMSOL and weak alternating
automata, and construct a type system for an automaton.  For a fixed
weak alternating automaton $\Aa$ we want to characterize the terms
whose B\"ohm trees are accepted by $\Aa$, i.e.\ the set $L(\Aa)$. The
characterization will be purely type theoretic
(cf.~Theorem~\ref{thm:main}).

Fix an automaton
$\Aa=\struct{Q,\S,q^0,\set{\delta_i}_{i\in\Nat},\rho}$. Let $m$ be the
maximal rank, i.e., the maximal value $\rho$ takes on $Q$.  For every
$0\leq k\leq m$ we write $Q_k=\set{q\in Q : \rho(q)=k}$ and
$\Qlk=\set{q\in Q: \rho(q)\leq k}$.



The type system we propose is obtained by allowing the use of
intersections inside simple types. This idea has been used by
Kobayashi~\cite{KobACM} to give a typing characterization for
languages of automata with trivial acceptance conditions.  We work
with, more general, weak acceptance conditions, and this will be
reflected in the stratification of types, and two fixpoint rules: greatest
fixpoint rule for even strata, and the least fixpoint rule for odd
strata.


First, we define the sets of intersection types. They are indexed by a
rank of the automaton and by a simple type. Note that every
intersection type will have a corresponding simple type; this is a
crucial difference with intersection types characterizing strongly
normalizing terms~\cite{BCD83}. Letting
$\Types^k_{A} = \bigcup_{0\leq l\leq k}\types^l_A$ we define\label{def:types}:
 $$\resizebox{\columnwidth}{!}{$\types_{o}^{k}= \set{q\in Q: \rho(q)= k},\,
   \types^k_{A\to B} = \set{T \to s : T \subseteq \Types^k_{A}\
     \text{and}\ s\in\types^k_{B}}\ .$}$$ The difference with simple
 types is that now we have a set constructor that will be interpreted
 as the intersection of its elements. This technical choice amounts to
 quotient types with respect to the associativity, the commutativity
 and the idempotency of the intersection operator. A nice consequence
 in our context is that the sets $\types^k_A$ and $\Types^k_A$ are
 finite. Notice also that the application of the intersection type
 operator to two sets
 of types is then represented by the union of those two sets.

\paragraph{\bf Example} Suppose that in $Q$ we have states $q_0,r_0,q_1$ with
ranks given by their subscripts. A type $\set{q_0,r_0}\incl
\Types^0_o$ will type terms whose B\"ohm tree is accepted both from
$q_0$ and from $r_0$.  A type $\set{\set{q_0,r_0}\to\set{q_1}}
\incl\types^1_{o\to o}$ will type terms that when given a term of type
$\set{q_0,r_0}$ produce a B\"ohm tree accepted from $q_1$. Observe
that, for example, $\set{\set{q_0,r_0}\to\set{q_1},\set{q_1}\to \set{q_1}}
\incl\Types^1_{o\to o}$ while $\set{\set{q_1},\set{q_1}\to \set{q_1}}$
is not an intersection type in our sense since the two types in the set
have different underlying simple types.\medskip



When we write $\types_{A}$ or $\Types_A$ we mean $\types^m_{A}$ and
$\Types^m_{A}$ respectively; where $m$ is the maximal rank used by the
automaton $\Aa$.


For $S\subseteq\Types^k_A$ and $T\subseteq\types^k_B$ we write $S\to
T$ for $\set{S\to t: t\in T}$. Notice that $S\to T$ is included in
$\types^{k}_{A\to B}$.

We now give subsumption rules that express the intuitive dependence
between types. So as to make the connection with the model
construction later, we have adopted an ordering of intersection types
that is dual to the usual one (the first rule can be derived from the
second and third one, but we find it more intuitive to explicitly
spell it out).  Usually in intersection types, the lower a type is in
the subsumption order, the less terms it can type. Here we take the
information order instead, the lower a type is in the subsumption
order, the less precise it is. As we said earlier, this choice is
motivated by the connection of types with models, 
 the information order gives us an isomorphism between the two, while
the usual choice would give us a duality between types and
models.
\begin{center}\small
  \begin{prooftree}
    S\subseteq T\subseteq Q%
    \justifies%
    S \tleq_o T
  \end{prooftree}
  \qquad
  \begin{prooftree}
    \forall s \in S, \exists t\in T,
    s\tleq_A t%
    \justifies%
    S\tleq_A T
  \end{prooftree}\smallskip
  \qquad
  \begin{prooftree}
    s=t%
    \justifies%
    s \tleq_o t
  \end{prooftree}
\qquad
  \begin{prooftree}
    T\tleq_A S\quad s\tleq_B t%
    \justifies%
    S\to s\tleq_{A\to B} T\to t%
  \end{prooftree}
\end{center}
 Given $S\incl\Types_{A\to B}$ and $T\incl
\Types_{A}$ we write $S(T)$ for the set $\set{t : (U\to t)\in S\text{
    and }  U\tleq T}$.\label{df:type-applicaiton}

The typing system presented in Figure~\ref{fig:type_system} derives
judgments of the form $\G\vdash M\geq S$ where $\G$ is an environment
containing all the free variables of the term $M$, and $S\incl \Types_A$
with $A$ the type of $M$.  As usual, an environment $\G$ is a finite
list $x_1\geq S_1,\dots, x_n\geq S_n$ where  $x_1,\dots,x_n$ are pairwise
distinct  variables of
type $A_i$, and $S_i\incl \Types_{A_i}$. We will use a functional
notation and write $\G(x_i)$ for $S_i$.  We shall also write $\G,x\geq
S$ for an extension of the environment $\G$ with the declaration
$x\geq S$.
%to denote an environment that declares the variables in the
%environment $\G$ and the variable $x$ with the assumption that $x$
%is not in the domain of $\G$.

The rules in the first row of Figure~\ref{fig:type_system} express
standard intersection types dependencies: the axiom, the intersection
rule and the subsumption rule.
The rules in the second line are specific to our
fixed automaton.  The third line
contains the usual rules for application and abstraction with the
caveat that the abstraction rule incorporates the stratification of
types with respect to ranks so that the types used in the judgment are
always well-formed.
The least
fixpoint rule in the next line is standard, it expresses that the
least fixpoint can be approximated by iterations started in the least
element: if we derive $\G\vdash \lambda x.M\geq \es\to T$ then  we
obtain that $\G\vdash Y x.M\geq T$, that can allow us to derive
$\G\vdash Y x.M\geq T'$ provided $\G\vdash \lambda x.M \geq T\to T'$ etc.
The greatest
fixpoint rule in the last line is more intricate. It is allowed only
on even strata.  If taken for $k=0$ the rule becomes the standard rule
for the greatest fixpoint as the set $T$ must be the empty set.
For $k>0$ the rule permits to incorporate
$T$ that is the result of the fixpoint computation on the lower
stratum. % Intuitively, since we consider judgments of the form $\G\vdash
% M\geq q$, the least fixpoint rule can be safely applied in any context,
% while the greatest fixpoint rule needs to be restricted as otherwise we
% would be back in the case of automata with trivial acceptance
% conditions from Theorem~\ref{thm:GFP-model}.

\begin{figure*}\small
  \centering
  \begin{prooftree}
    \justifies%
    \G, x\geq S \vdash x\geq S
  \end{prooftree}
\quad
\begin{prooftree}
  \G\vdash M\geq S%
  \quad
  \G\vdash M\geq T%
  \justifies%
  \G\vdash M\geq S\cup T%
\end{prooftree}
\quad
\begin{prooftree}
  \G\vdash M\geq S%
  \quad%
  T\tleq S%
  \justifies
  \G\vdash M\geq T%
\end{prooftree}


\bigskip


\begin{prooftree}
\ %
  \justifies%
  \G \vdash c \geq \set{q: \delta_0(q,c) \neq \es}
\end{prooftree}
\quad
\begin{prooftree}
  (S_1,\dots,S_i) \in \delta_i(a,q)%
  \justifies%
  \G \vdash a \geq \set{S_1 \to \dots \to S_i \to q}
\end{prooftree}

\bigskip

\begin{prooftree}
  \G \vdash M \geq S %
  \quad%
  \G \vdash N \geq T
  \justifies%
  \G\vdash MN \geq S(T)%
\end{prooftree}
\quad
\begin{prooftree}
  S\subseteq\Types^{k},\, T\subseteq \types^k%
  \quad%
  \G, x\geq S \vdash M\geq T%
  \justifies%
  \G \vdash  \lambda x. M \geq S \to T%
\end{prooftree}

\bigskip

\begin{prooftree}
    \G \vdash (\lambda x. M)\geq S%
  \quad%
  \G\vdash (Y x .M) \geq T%
  \justifies%
  \G \vdash Y x.M\geq S(T)%
  \using Y\,\mathit{odd}%
\end{prooftree}

\bigskip

\begin{prooftree}
  S \subseteq \types^{2k}_{A},\quad%
  T\subseteq \Types^{2k-1}_{A},\quad%
  \G\vdash \lambda x.M\geq (S\cup T) \to S%
  \quad%
  \G\vdash Y x.M\geq T%
  \justifies%
  \G \vdash Y x.M\geq S\cup T%
  \using Y\,\mathit{even}%
\end{prooftree}
\caption{Type system}\label{fig:type_system}
\end{figure*}

Our main result says that the typing in
this system is equivalent to accepting with our fixed weak
alternating automaton.
\begin{thm}\label{thm:main}
  For every closed term $M$ of type $o$ and every state $q$ of $\Aa$:
  the judgment
  $\vdash M\geq q$ is derivable iff $\Aa$ accepts $BT(M)$ from $q$.
\end{thm}
Since there are finitely many types, this typing system is decidable.
As we will see in the following example, this type system allows us to
prove in a rather simple manner properties of B\"ohm trees that are
beyond the reach of trivial automata.  Compared to Kobayashi and Ong
type system~\cite{kobayashi09:_type_system_equiv_to_modal} and to
Tsukada and Ong type system~\cite{TsuOng14}, the
fixpoint typing rules we propose do not refer to an external parity
game.
%avoid the use of an external solver for a parity game. 
Our type system does not require \emph{flagged
  types}, and is
on the contrary based on a standard treatment of free variables. In
the example below we use fixpoint rules on terms of order $2$.


In order to prove Theorem~\ref{thm:main} we will need to formulate and
prove a more general statement that concerns terms of all types
(Theorem~\ref{thm:types_correctness_completeness}). To describe the
properties of the type system in higher types, we will construct a
model from our fixed automaton $\Aa$, and show
(Theorem~\ref{thm:model-correct}) that the model recognizes $L(\Aa)$
in the sense of Definition~\ref{df:recognizability}. Then
Theorem~\ref{thm:types_correctness_completeness} will say that the
type system reflects the values of the terms in the model.

Due to the symmetries in weak alternating automata, and in the model
we are going to construct, we will obtain also a dual type system. This
system can be used to show that the B\"ohm tree of a term is not
accepted by the automaton.


\begin{figure*}
  \centering
   \begin{prooftree}
    S\subseteq T\subseteq Q%
    \justifies%
    S \tgeq_o T
  \end{prooftree}
  \qquad
  \begin{prooftree}
    \forall s \in S, \exists t\in T,
    s\tgeq_A t%
    \justifies%
    S\tgeq_A T
  \end{prooftree}
  \qquad
  \begin{prooftree}
    s=t%
    \justifies%
    s \tgeq_o t
  \end{prooftree}
  \qquad
  \begin{prooftree}
    T\tgeq_A S\quad s\tgeq_B t%
    \justifies%
    S\to s\tgeq_{A\to B} T\to t%
  \end{prooftree}

  \medskip

%   \begin{prooftree}
%     \justifies%
%     \G, x \ngeq S \vdash x \ngeq S
%   \end{prooftree}
% \quad
% \begin{prooftree}
%   \G\vdash M \ngeq S%
%   \quad
%   \G\vdash M \ngeq T%
%   \justifies%
%   \G\vdash M \ngeq S\cup T%
% \end{prooftree}
% \quad
% \begin{prooftree}
%   \G\vdash M \ngeq S%
%   \quad%
%   T \tgeq  S%
%   \justifies
%   \G\vdash M \ngeq T%
% \end{prooftree}


% \bigskip

\begin{prooftree}
\ %
  \justifies%
  \G \vdash c \geq \set{q: \delta_o(q,c)=\es}
\end{prooftree}
\quad
\begin{prooftree}
  \forall (S_1,S_2)\in\delta(a,q), (T_1\cap S_1)\cup (T_2\cap S_2)\neq \es%
  \justifies%
  \G \vdash a \ngeq T_1 \to T_2 \to q%
\end{prooftree}

\medskip

\begin{prooftree}
  \G \vdash M \ngeq S %
  \quad%
  \G \vdash N \ngeq T
  \justifies%
  \G\vdash MN \ngeq S(T)%
\end{prooftree}
\quad
\begin{prooftree}
  S\in\Types^{k},\, T\subseteq \types^k%
  \quad%
  \G, x\ngeq S \vdash M\ngeq T%
  \justifies%
  \G \vdash  \lambda x. M \ngeq S \to T%
\end{prooftree}


\medskip

\begin{prooftree}
  S \subseteq \types^{2k+1}_{A},\quad%
  T\in \Types^{2k}_{A},\quad%
  \G\vdash \lambda x.M\ngeq (S\cup T) \to S%
  \quad%
  \G\vdash Y x.M\ngeq T%
  \justifies%
  \G \vdash Y x.M\ngeq S\cup T%
  \using Y\,\mathit{odd}%
\end{prooftree}


\medskip

\begin{prooftree}
  \G \vdash (\lambda x. M)\ngeq S%
  \quad%
  \G\vdash (Y x .M) \ngeq T%
  \justifies%
  \G \vdash Y x.M \ngeq S(T)%
  \using Y\,\mathit{even}%
\end{prooftree}

\caption{Dual type system}\label{fig:dual_type_system}

\end{figure*}


The dual type system is presented in Figure~\ref{fig:dual_type_system}
on page~\pageref{fig:dual_type_system}. The notation is as before but
we now define $S(T)$ to be $\set{s : U\to s\in S\land U\tgeq T}$. The
rules for application, abstraction and variable do not change.  By duality we
obtain:
\begin{cor}
  For every closed term $M$ of type $o$ and every state $q$ of $\Aa$:
  judgment $\vdash M\ngeq q$ is derivable iff $\Aa$ does not accept $BT(M)$ from $q$.
\end{cor}
So the two type systems together allow us to derive both positive and
negative information about a program.



We finish this section with two moderate size examples of typing
derivations.

\paragraph{\bf Example}
Take a signature consisting of two constants $c:o$ and $a:o\to o$. We
consider an extremely simple weak alternating automaton with just
one state $q$ of rank $1$ and transitions:
\begin{equation*}
  \delta(q,a)=\set{q}\qquad \delta(q,c)=\es\ .
\end{equation*}
This automaton accepts the finite sequences of $a$'s ending in $c$.
Observe that these transition rules give us typing axioms
\begin{center}
  \begin{prooftree}
    \
    \justifies
    \vdash a\geq \set{q}\to q
  \end{prooftree}
\qquad
  \begin{prooftree}
    \
    \justifies
    \vdash c\geq q
  \end{prooftree}
\end{center}
Notice that we omit some set
parenthesis over singletons; so for example we write $c\geq q$ instead
of $c\geq \set{q}$. In this example we will still keep the parenthesis
to the left of the arrow to emphasize that we are in our type system, and not in
simple types. In the next example we will omit them too.

First, let us look at a term $G_1\equiv \lambda f^{o\to
  o}\lambda x^o.\ f(f x)$. It has a simple type $\tau_1\equiv (o\to o)\to
o \to o$. The judgment $\vdash G_1\geq \g_1$ is derivable in our
system; where $\g_1\equiv\set{\set{q}\to q}\to\set{q}\to q$.
\begin{center}
  \begin{prooftree}
  \begin{prooftree}
    \G\vdash f\geq\set{q}\to q
    \quad
  \begin{prooftree}
    \G\vdash f\geq\set{q}\to q
    \quad
    \G\vdash x\geq q
    \justifies
    \G\vdash fx\geq q
  \end{prooftree}
  \justifies
    \G\vdash f(fx)\geq q
  \end{prooftree}
\justifies
\vdash \lambda f\lambda x.\ f(f x) \geq \g_1
\end{prooftree}
\end{center}
here $\G\equiv f\geq \set{q}\to q,\ x\geq q$.

Consider now $G_2\equiv \lambda f^{\tau_1}\lambda x^{o\to o}.\ f(f x)$. We have
that $G_2$ is of type $\tau_2\equiv \tau_1\to\tau_1$. A derivation very
similar to the above
will show $\vdash G_2\geq \g_2$ where $\g_2\equiv \set{\g_1}\to\g_1$.

Then by induction we can define $G_i\equiv \lambda f^{\tau_{i-1}}\lambda
x^{\tau_{i-2}}.\ f(f x)$ that is of a type $\tau_i\equiv
  \tau_{i-1}\to\tau_{i-1}$. Still a similar derivation as above will show $\vdash
  G_i\geq \g_i$ where $\g_i\equiv \set{\g_{i-1}}\to\g_{i-1}$.

One use of application rule then shows that $G_i G_{i-1}\geq \g_{i-1}$:
\begin{center}
  \begin{prooftree}
    \vdash G_i\geq \set{\g_{i-1}}\to\g_{i-1}
    \quad
    \vdash G_{i-1}\geq \g_{i-1}
    \justifies
    \vdash G_i G_{i-1}\geq \g_{i-1}
  \end{prooftree}
\end{center}

In consequence, we can construct by induction a derivation of
\begin{equation*}
  \vdash G_iG_{i-1}\dots G_1 a c\geq q
\end{equation*}
This derivation proves that the B\"ohm tree of $G_iG_{i-1}\dots G_1 a
c$ is a sequence of $a$'s ending in $c$. While the length of this sequence
is a tower of exponentials in the height $i$, the typing derivation we have
constructed is linear in $i$ (if types are represented
succinctly). This simple example, already analyzed in~\cite{KobACM}, shows the power of modular
reasoning provided by the typing approach.
 We should note though that if
the initial automaton had two states, the number of
potential types would also be  roughly the tower of exponentials
in $i$. Due to the complexity bounds~\cite{terui_semantic_evaluation},
there are terms and automata for which there is no small
derivation. Yet one can hope that in many cases a small derivation
exists. For example, if we wanted to show that the length of the
sequence is even then the automaton would have two states but the
derivation would be essentially the same.

\paragraph{\bf Example} Consider the term $M=(YF.N) a$ where $N=\lambda
g.g(b(F(\lambda x. g(g\, x))))$. As we have seen on page~\pageref{ex:one},
$BT(M) = ab a^2 b a^4 b\dots a^{2^n}b \dots$. We show with typing that
there are infinitely many occurrences of $b$ in $BT(M)$. To this end
we take an automaton having states $Q=\set{q_1,q_2}$, and working over the
signature containing $a$ and $b$.  The transitions of the automaton are:
  $$\delta(q_1, a)=\set{q_1}, \quad  \delta(q_2, a) = \set{q_1,q_2},
  \quad \delta(q_1, b)   =\es, \quad
  \delta(q_2, b) = q_2\ .$$
The ranks of states are indicated by their subscripts. Starting with
state $q_2$, the automaton only accepts sequences that contain
infinitely many $b$'s.
 So our goal is to derive $\vdash
(YF.N)a\geq q_2$.  First observe that from the definition of the
transitions of the automaton we get axioms:
\begin{center}\small
%\resizebox{\columnwidth}{!}{
\begin{prooftree}
\
\justifies
\vdash a\geq q_1\to q_1
\end{prooftree}
\quad
\begin{prooftree}
\
\justifies
\vdash a\geq \set{q_1,q_2}\to q_2
\end{prooftree}
\quad
\begin{prooftree}
\
\justifies
\vdash b\geq \es\to q_1
\end{prooftree}
\quad
\begin{prooftree}
\
\justifies
\vdash b\geq q_2\to q_2
\end{prooftree}
%}
\end{center}
Looking at the typings of $a$, we can see that we will get our desired
judgment from the application rule if we prove:
\begin{equation*}\small
  \vdash YF.N\geq S\qquad\text{where $S$ is $\set{q_1\to
      q_1,\set{q_1,q_2}\to q_2}\to  q_2$.}
\end{equation*}
To this end, we apply the subsumption rule and the greatest fixpoint rule:
\begin{center}\small
    \begin{prooftree}
      \begin{prooftree}
          \vdash \lambda F.N\geq (S\cup T)\to S
        \quad
          \vdash YF.N\geq T
        \justifies%
        \vdash YF.N \geq S\cup T\using Y\,\textit{even}
      \end{prooftree}
      \justifies%
      \vdash YF.N \geq S
    \end{prooftree}
\qquad
\text{where $T=\set{(q_1\to q_1)\to q_1}$}
\end{center}
The derivation of the top right judgment uses the least fixpoint
rule:

\begin{center}
  \small
  \begin{prooftree}
    \begin{prooftree}
      \begin{prooftree}
        \begin{prooftree}
          \justifies
          g\geq q_1\to q_1 \vdash g\geq q_1\to q_1
        \end{prooftree}
        \quad
          g\geq q_1\to q_1 \vdash b(F(\lambda x.g(g\,x)))\geq q_1
        \justifies%
        g\geq q_1\to q_1 \vdash g(b(F(\lambda x.g(g\,x))))\geq q_1
      \end{prooftree}
      \justifies%
      \vdash \lambda F\lambda g.g(b(F(\lambda x.g(g\,x)))) \geq \es \to(q_1\to q_1 )\to
      q_1
    \end{prooftree}
    \justifies%
    \vdash YF. N \geq (q_1\to q_1)\to q_1
    \using Y\,\mathit{odd}%
  \end{prooftree}
\end{center}
We have displayed only one of the two premises of the $Y odd$ rule
since the other is of the form $\geq \es$ so it is vacuously true.
The top right judgment is derivable directly from the axiom on $b$.
The derivation of the remaining judgment $\vdash \lambda F.N\geq (S\cup T)\to S$ is as
follows.
\begin{center}\small
  \begin{prooftree}
    \begin{prooftree}
      \begin{prooftree}
        \justifies
        \G \vdash g\geq \set{q_1,q_2}\to q_2
      \end{prooftree}

      \quad
      \G \vdash b(F(\lambda x. g(g\,x))) \geq q_1,q_2
      \justifies%
      \G \vdash  g(b(F(\lambda x. g(g\,x)))) \geq q_2
    \end{prooftree}
    \justifies%
    \vdash \lambda F \lambda g. g(b(F(\lambda x. g(g\,x)))) \geq (S\cup T)\to S
  \end{prooftree}
\end{center}
where $\G$ is $F\geq S\cup T, g\geq \set{q_1\to q_1,\set{q_1,q_2}\to
  q_2}$. So the upper left judgment is an axiom. The other judgment
on the top is an abbreviation of two judgments: one to show $\geq
q_1$ and the other one to show $\geq q_2$. These two judgments are proved
directly using application and intersection rules.




%%% Local Variables:
%%% mode: latex
%%% TeX-master: "m"
%%% End:

%  LocalWords:  wMSOL Kobayashi fixpoint BT fx iG subterms YF typings
%  LocalWords:  subsumption exponentials Ong


==> type-system2.tex <==
We are now in a position to show that our type system from
Figure~\ref{fig:type_system} can reason about the values of $\lambda
Y$-terms in a stratified model, cf.\
Theorem~\ref{thm:types_correctness_completeness} below. Thanks to
Theorem~\ref{thm:model-correct} this means that the type system can
talk about the acceptance of the B\"ohm tree of a term by the automaton.
This implies the soundness and completeness of our type system,
Theorem~\ref{thm:main}.

Throughout this section we work with a fixed signature
$\S$ and a fixed weak alternating automaton
$\Aa=\struct{Q,\S,q^0,\delta_o,\delta_{o^2\to o},\rho}$.  As in the
previous section, for the sake of the simplicity of notations we will
assume that the
constants in the signature are of type $o$ or $o\to o\to o$.
We will also prefer the notation $Y x.M$ to $Y(\lambda x. M)$.


% The type system we introduced in Section~\ref{sec:type-system} can be
% understood as means for reasoning about the values of a term in a
% model. Indeed, we will show that types can denote all elements in the
% model (Lemma~\ref{lem:sem_representations_with_types}).  This follows
% Abramsky's idea of domains in logical
% form~\cite{abramsky91:_domain_theor_logic_form} further adapted to the
% typed setting in~\cite{salvati12:logical_relation}.% For
% this we first give a syntactic representation of elements of the model
% akin to intersection types.  The sets $\types^{k}_{A}$ and
% $\Types^k_A$ are defined by induction the structure of $A$:

The arrow constructor in types will be interpreted as a step function
in the model.  Step functions are  particular monotone functions from a
lattice $\Ll_1$ to a lattice $\Ll_2$. For later use we also define
co-step functions.
For $d$ in $\Ll_1$ and $e$ in $\Ll_2$, the \emph{step function}
$d\step e$ and the \emph{co-step function} $d\costep g$ are defined
by:
\begin{align*}
  (d\step e)(h) =& \left\lbrace
    \begin{array}{l}
      e \text{ when } d\leq h\\
      \bot \text{ otherwise}
    \end{array}
    \right.
&
    (d\costep e)(h) =& \left\lbrace
      \begin{array}{l}
        e \text{ when } h\leq d\\
        \top \text{ otherwise\ .}
      \end{array}
      \right.
\end{align*}
To emphasize that we work in $\Dd^k$ we will sometimes write $d\step^k e$ and
$d\costep^k e$.


Types introduced on page~\pageref{def:types} can be meaningfully
interpreted at every level of the model. So $\tint{t}^k$ will denote
the interpretation of $t$ in $\Dd^k$ defined as follows.
\begin{align*}
  \tint{q}^{k} &= \set{q} \text{ if }\rho(q)\leq k,\,\es \text{ otherwise}\\
% \begin{cases}
%     \set{q} & \text{if the rank of $q$ is at most $l$}\\
%     \es & \text{otherwise}
%   \end{cases}\\
  \tint{S}^k & = \Lor\set{\tint{t}^k : t\in S}\qquad\text{for $S\incl \Types_A$}\\
  \tint{T\to s}^k&= \tint{T}^k\step\tint{s}^k\qquad\text{for $(T\to s)\in \Types_A$}
\end{align*}


Directly from the definition we have $\tint{S_1\cup S_2}^k =
\tint{S_1}^k\vee \tint{S_2}^k$, and  $\tint{S\to T}^{k} =
\tint{S}^{k}\step^k \tint{T}^{k}$.


The next lemma summarizes basic facts about the interpretation of
types. Recall that the application operation  $S(T)$ on types
(cf. page~\pageref{df:type-applicaiton}) means $\set{t : (U\to t)\in S\land
  U\tleq T}$. The proof of the lemma uses
Corollaries~\ref{cor:up-down} and~\ref{coro:galois_connections}.
\begin{lem}
  \label{lem:types_and_level_prop}
  For every type $A$, if $S\incl\Types_A$ and $k\leq m$ we have:
  $\tint{S}^k=\tint{S\cap \Types^k_A}^k$, $\tint{S\cap
    \Types^k_A}^{k+1} = (\sem{S}^k_A)\upinf$ and
  $\tint{S}^k=(\tint{S}^{k+1})\down$. % For every $S\incl \Types^k_{A\to
  %   B}$ and $T\incl \Types^k_{A}$ we have:
  % $\sem{S(T)}^k=\sem{S}^k(\sem{T}^k)$.
\end{lem}
\begin{proof}
  Consider the first statement.
  Since $\tint{S}^k = \Lor\set{\tint{t}^k : t\in S}$ it is sufficient
  to show that $\tint{t}^k=\bot^k_A$ for $t\not\in\Types^k_A$. We do it by
  induction on the type $A$.

  Suppose that $t\in\types^l_A$ for $l>k$.
  For the type $o$ it follows directly from the definition that
  $\tint{t}^k=\es$. For $A$ of the form $B\to C$ we know that $t$ is
  of the form $T\to s$ with $T\incl \Types^l_B$ and $s\in\types^l_C$.
  By induction assumption $\tint{s}^k=\bot^k_C$. We get $\tint{T\to
    s}^k=\tint{T}^k\step^k\tint{s}^k=\tint{T}^k\step^k\bot_C=\bot^k_{B\to
    C}$.

  We give the proof of the second statement, the proof of the third is
  analogous.
  We prove the result only for elements of $\types^k_A$ as the more
  general one is a direct consequence of that particular case.
  The proof is by induction on $A$. The base case is obvious. For $A$
  of the form $B\to C$ we have $\tint{T\to s}^{k+1}$ is by definition
  $\tint{T}^{k+1}\step^{k+1}\tint{s}^{k+1}$ which by induction
  hypothesis is $(\tint{T}^k)\upinf\step^{k+1}(\tint{s}^k)\upinf$.
  We will be done if we show that for every $f\in \Dd^k_B$ and
  $g\in\Dd^k_C$:
  \begin{equation*}
    f\upinf\step^{k+1}g\upinf=(f\step^k g)\upinf\ .
  \end{equation*}
  Given $e$ in $\Dd^{k+1}_{B}$,
  by Corollary~\ref{cor:up-down}, we have $(f\step^{k}
  g)\upinf(e)$ is equal to $((f\step^k g)(e\down))\upinf$, and
  therefore:
  \begin{equation*}
  (f\step^{k}  g)\upinf(e) =
  \begin{cases}
      g\upinf & \text{ if } f\leq e\down, \\
      \bot^{k+1}_C&  \text{ otherwise}.
  \end{cases}
  \end{equation*}
  Since $f\leq e\down$ iff $ f\upinf\leq e$, by
  Corollary~\ref{coro:galois_connections}, this  proves the desired
  equality.%\todo{Fourth statement}
\end{proof}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Directly from the definition we have $\tint{S_1\cup S_2}^l =
% \tint{S_1}^l\vee \tint{S_2}^l$, and  $\tint{S\to T}^{l} =
% \tint{S}^{l}\step^l \tint{T}^{l}$.
%
%
% The next lemma summarizes basic facts about the interpretation of
% types. Recall that the application operation  $S(T)$ on types
% (cf. page~\pageref{df:type-applicaiton}) means $\set{t : (U\to t)\in S\land
%   U\tleq T}$. The proof of the lemma uses
% Corollaries~\ref{cor:up-down} and~\ref{coro:galois_connections}.
% \begin{lem}
%   \label{lem:types_and_level_prop}
%   For every type $A$, if $S\incl\Types_A$ and $k\leq m$ we have:
%   $\tint{S}^k=\tint{S\cap \Types^k_A}^k$, $\tint{S\cap
%     \Types^k_A}^{k+1} = (\sem{S}^k_A)\upinf$ and
%   $\tint{S}^k=(\tint{S}^{k+1})\down$. For every $S\incl \Types^k_{A\to
%     B}$ and $T\incl \Types^k_{A}$ we have:
%   $\sem{S(T)}^k=\sem{S}^k(\sem{T}^k)$.
% \end{lem}
% \begin{proof}
%   Consider the first statement.
%   Since $\tint{S}^l = \Lor\set{\tint{t}^l : t\in S}$ it is sufficient
%   to show that $\tint{t}^k=\bot^k_A$ for $t\not\in\Types^k_A$. We do it by
%   induction on the type $A$.
%
%   Suppose that $t\in\types^l_A$ for $l>k$.
%   For type $0$ it follows directly from the definition that
%   $\tint{t}^k=\es$. For $A$ of the form $B\to C$ we know that $t$ is
%   of the form $T\to s$ with $T\incl \Types^k_B$ and $s\in\types^l_C$.
%   By induction assumption $\tint{s}^k=\bot^k_C$. We get $\tint{T\to
%     s}^k=\tint{T}^k\step^k\tint{s}^k=\tint{T}^k\step^k\bot_C=\bot^k_{B\to
%     C}$.
%
%   We give the proof of the second statement, the proof of the third is
%   analogous.
%   We prove the result only for elements of $\types^k_A$ as the more
%   general one is a direct consequence of that particular case.
%   The proof is by induction on $A$. The base case is obvious. For $A$
%   of the form $B\to C$ we have $\tint{T\to s}^{k+1}$ is by definition
%   $\tint{T}^{k+1}\step^{k+1}\tint{s}^{k+1}$ which by induction
%   hypothesis is $(\tint{T}^k)\upinf\step^{k+1}(\tint{s}^k)\upinf$.
%   We will be done if we show that for every $f\in \Dd^k_B$ and
%   $g\in\Dd^k_C$:
%   \begin{equation*}
%     f\upinf\step^{k+1}g\upinf=(f\step^k g)\upinf\ .
%   \end{equation*}
%   Given $e$ in $\Dd^{k+1}_{B}$,
%   by Corollary~\ref{cor:up-down}, we have $(f\step^{k}
%   g)\upinf(e)$ is equal to $((f\step^k g)(e\down))\upinf$, and
%   therefore:
%   \begin{equation*}
%   (f\step^{k}  g)\upinf(e) =
%   \begin{cases}
%       g\upinf & \text{ if } f\leq e\down, \\
%       \bot^{k+1}_C&  \text{ otherwise}.
%   \end{cases}
%   \end{equation*}
%   Since $f\leq e\down$ iff $ f\upinf\leq e$, by
%   Corollary~\ref{coro:galois_connections}, this  proves the desired
%   equality.\todo{Fourth statement}
%   \qed
%
% \end{proof}
%
%
%
%
% \begin{cor}
%   For every $k\leq m$ and every $S\in\Types_A$ we have:
%   $\tint{S}^k=(\tint{S}^{k+1})\down$.
% \end{cor}
% We can now show that every element of $\Dd^k_{A}$ is representable by
% a type. For this we use $\bar{(\cdot)}$ operation (cf.\ Definition~\ref{df:bar}).
%
%
% \begin{lem}
%   \label{lem:sem_representations_with_types}
%   For every $k\leq m$ and  every type $A$. For  every $d$ in $\Dd^k_{A}$
%   there is $S\incl\Types^k_{A}$ so that $\tint{S}^{k} = d$, and there
%   is $S'\incl \types^k_A$ so that $\tint{S'}^{k} = \bar d$.
% \end{lem}
% \begin{proof}
%     We proceed by induction on $k$.
%
%   The case where $k=0$ has been proved in~\cite{SalWalTLCA}.
%
%   For the case $k >0$, as we have seen with
%   Lemma~\ref{lem:Nn_k_decomposition}, that $f = (f\down)\upinf \vee
%   \overline{f}$. From the induction hypothesis there is $S_1\incl
%   \Types^{k-1}_A$ such that $\tint{S_1}^{k-1}=f\down$. By
%   Lemma~\ref{lem:types_and_level_prop} we get $\tint{S_1}^k=(f\down)\upinf$.
%
%   It remains to describe $\overline{f}$ with types from $\types^k_{B\to
%     C}$. Take $d\in\Dd^k_B$ and recall that $\bar f
%   (d)=\bar{f(d)}$. By induction hypothesis we have $S_d\incl
%   \Types^k_B$ and $S_{\bar{f(d)}}\incl \types^k_{C}$ such that
%   $\tint{S_d}^k=d$ and $\tint{S_{\bar{f(d)}}}^k=f(d)$. So the set of
%   types $S_d\to S_{\overline{f(d)}}$ is included in $\types^k_{B\to C}$ and
%   $\tint{S_d\to S_{\overline{f(d)}}}=d\step^k\bar f(d)$. It remains to take
%   $S_2=\bigcup\set{S_d | d\in \Dd^k_B}$. We can conclude that $S_2\incl
%   \types^k_A$ and $\tint{S_2}^k=\bar f$. Therefore $\tint{S_1\cup
%     S_2}^k=f$.
%   \qed
% \end{proof}
%
%
% \begin{lem}
%   \label{lemma:ordering_correct_complete}
%   For every $k$, $A$, and $S,T\incl\Types^k_A$:\quad
%   $\tint{S}^{k}\leq\tint{T}^k$ iff $S\tleq_A T$.
% \end{lem}
% \begin{proof}
%   This lemma is a consequence of the fact that for each $k$, $\Dd_k$
%   can be embedded in the monotone model generated by $\Pp(\Qlk)$ and
%   that according to~\cite{salvati12:logical_relation}, the ordering on
%   intersection types simulate the one in monotone models.\qed
% \end{proof}
%
%
%
% \begin{lem}
%   \label{lem:type_application_is_sem_application}
%   For $S\incl\Types^k_{A\to B}$ and $T\incl\Types^k_A$,  we have:
%   $\tint{S(T)}^k = \tint{S}^{k}(\tint{T}^k)$.
% \end{lem}
%
% \begin{proof}
%   Immediate.\qed
% \end{proof}
%
%The type system is presented in Figure~\ref{fig:type_system}.
%


Actually every element of $\Dd^k$ is the image of some type via $\tint{\cdot}^k$: types
are syntactic representations of the model.
For this we use $\bar{(\cdot)}$ operation (cf.\ Definition~\ref{df:bar}).


\begin{lem}
  \label{lem:sem_representations_with_types}
  For every $k\leq m$, every type $A$ and  every $d$ in $\Dd^k_{A}$
  there is $S\incl\Types^k_{A}$ so that $\tint{S}^{k} = d$, and there
  is $S'\incl \types^k_A$ so that $\tint{S'}^{k} = \bar d$.
\end{lem}
\begin{proof}
    We proceed by induction on $k$.

  The case where $k=0$ has been proved in~\cite{SalWalTLCA}.

  For the case $k >0$, as we have seen with
  Lemma~\ref{lem:Nn_k_decomposition}, that $f = (f\down)\upinf \vee
  \overline{f}$. From the induction hypothesis there is $S_1\incl
  \Types^{k-1}_A$ such that $\tint{S_1}^{k-1}=f\down$. By
  Lemma~\ref{lem:types_and_level_prop} we get $\tint{S_1}^k=(f\down)\upinf$.

  It remains to describe $\overline{f}$ with types from $\types^k_{B\to
    C}$. Take $d\in\Dd^k_B$ and recall that $\bar f
  (d)=\bar{f(d)}$. By induction hypothesis we have $S_d\incl
  \Types^k_B$ and $S_{\bar{f(d)}}\incl \types^k_{C}$ such that
  $\tint{S_d}^k=d$ and $\tint{S_{\bar{f(d)}}}^k=f(d)$. So the set of
  types $S_d\to S_{\overline{f(d)}}$ is included in $\types^k_{B\to C}$ and
  $\tint{S_d\to S_{\overline{f(d)}}}=d\step^k\bar f(d)$. It remains to take
  $S_2=\bigcup\set{S_d \to S_{\overline{f(d)}}\mid d\in \Dd^k_B}$. We can
  conclude that $S_2\incl
  \types^k_A$ and $\tint{S_2}^k=\bar f$. Therefore $\tint{S_1\cup
    S_2}^k=f$.
\end{proof}

Not only can type represent every element of the model, but also the
subsumption rule exactly represents the partial order of the model.

\begin{lem}\label{lem:ordering_correct_complete}
  For each $k$, $A$, $S$ and $T$ in $\Types^k_A$, we have that
  $\tint{S}^{k}\leq\tint{T}^k$ iff $S\tleq_A T$.
\end{lem}
\begin{proof}
  This is a consequence of the fact that for each $k$, $\Dd_k$
  can be embedded in the monotone model generated by $\Pp(\Qlk)$ and
  that according to~\cite{salvati12:logical_relation}, the ordering on
  intersection types simulate the one in monotone models.
\end{proof}

An immediate consequence is that the application that we defined at
the level of type simulates the application in the model.

\begin{lem}
  \label{lem:type_application_is_sem_application}
  For $S\incl\Types^k_{A\to B}$ and $T\incl\Types^k_A$,  we have:
  $$\tint{S(T)}^k = \tint{S}^{k}(\tint{T}^k)\ .$$
\end{lem}

\begin{proof}
  By definition
  $S(T) = \set{t \mid (U\to t)\in S\text{ and } U\tleq T}$,
  but
  $\tint{S}^k = \bigvee \set{\tint{U\to t}^k\mid U\to t\in S} =
  \bigvee \set{\tint{U}^k \step^k \tint{t}^k\mid U\to t\in S}$ and
  thus
  $\tint{S}^{k}(\tint{T}^k) = \bigvee \set{\tint{t}^k\mid U\to t\in S
    \text{ and } \tint{U}^k\leq \tint{T}^k}$. From
  Lemma~\ref{lem:ordering_correct_complete}, $U\tleq T$
  iff $\tint{U}^k \leq \tint{T}^k$
  and we then obtain the expected idendity:
  $\tint{S}^{k}(\tint{T}^k) = \set{t \mid (U\to t)\in S\text{ and }
    U\tleq T} = S(T)$.
\end{proof}


The next theorem is the
main technical result of the paper. It says
that the type system can derive all lower-approximations of the meanings of
terms in the model. For an environment $\G$, we write
$\sem{\G}^k$ for the valuation such that $\sem{\G}^k(x) =
\tint{\G(x)}^k$.

\begin{thm}
  \label{thm:types_correctness_completeness}
  For $k=0,\dots,m$ and $S\subseteq \Types^k$:
  \begin{equation*}
    \text{$\sem{M}^k_{\sem{\G}^k}\geq \tint{S}^k$\quad
  iff\quad $\G\vdash M\geq S$ is derivable.}
  \end{equation*}


\end{thm}

The above theorem implies Theorem~\ref{thm:main} stating soundness and
completeness of the type system. Indeed, let us take a closed term $M$
of type $o$, and a state $q$ of our fixed automaton
$\Aa$. Theorem~\ref{thm:model-correct} tells us that $\sem{M}=\Aa(M)$;
where $\Aa(M)$ is the set of states from which $\Aa$ accepts $BT(M)$. So
$\vdash M\geq q$ is derivable iff $\sem{M}\supseteq\set{q}$ iff $q\in
\Aa(M)$.

The theorem is proved by the following two lemmas.
% \begin{cor}
%   For every closed term $M$ of type $o$ and every state $q\in Q$:
%   $\vdash M\geq q$ is derivable iff $\Aa$ accepts $BT(M)$ from $q$.
% \end{cor}

\begin{lem}
%  \label{lemma:types_correctness}
  If $\Gamma\vdash M\geq S$ is derivable, then for every $k\leq m$:
  $\sem{M}^k_{\sem{\G}^k}\geq \tint{S}^k$.
\end{lem}
\begin{proof}
  This proof is done by a simple induction on the structure of the
  derivation of $\G\vdash M\geq S$.  For most of the rules, the
  conclusion follows immediately from the induction hypothesis (using
  the
  Lemmas~\ref{lem:types_and_level_prop},~\ref{lem:ordering_correct_complete}
  and~\ref{lem:type_application_is_sem_application}). We shall only
  treat here the case of the rules $Y\ \mathit{odd}$ and $Y\
  \mathit{even}$.

  In the case of $Y\ \mathit{odd}$, when we derive $\G\vdash Y x.M\geq
  S(T)$ from $\G\vdash \lambda x.M\geq S$ and $\G\vdash Y x.M\geq T$,
  the induction hypothesis gives that for
  every $k$, $\sem{\lambda x. M}^k_{\sem{\G}^k}\geq \tint{S}^k$
  and $\sem{Y x. M}^k_{\sem{\G}^k}\geq \tint{T}^k$.
  Therefore $\sem{Yx.M}^k_{\sem{\G}^k} = \sem{(\lambda x.M)(Y
    x.M)}^k_{\sem{\G}^k} \geq \tint{S}^k(\tint{T}^k) = \tint{S(T)}^k$, using
  Lemma~\ref{lem:type_application_is_sem_application}.

  In the case of $Y\ \mathit{even}$ we consider the case $k=2l$.
  Let $\nu_{k-1}$ stand for $\sem{\G}^{k-1}$ and $\nu_{k}$ for
  $\sem{\G}^{k}$.

  By induction hypothesis we have $\sem{Y x.M}^{k-1}_{\nu_{k-1}}\geq
  \tint{T}^{k-1}$. Since Lemma~\ref{cor:L-on-terms} implies $(\sem{Y
    x.M}^{k-1}_{\nu_{k-1}},\sem{Y x.M}^{k}_{\nu_{k}})\in \Ll^k$, we have
  $\sem{Y x.M}^{k}_{\nu_{k}}\geq (\tint{T}^{k-1})\upinf$ by
  Lemma~\ref{lem:galloi_connections}. By Lemma~\ref{lem:types_and_level_prop} we
  know $(\tint{T}^{k-1})\upinf=\tint{T}^k$. In consequence we have
  \begin{equation*}
      \sem{\lambda x.M}^k_{\nu_k}(\tint{T}^k)\geq \tint{T}^k.
  \end{equation*}
  Also by induction hypothesis we have $\sem{\lambda x. M}^k_{\nu_k}\geq
  \tint{(S\cup T)\to S}^k$. This means that $\sem{\lambda
    x.M}^k_{\nu_k}(\tint{S\cup T}^k)\geq \tint{S}^k$. Put together
  with what we have concluded about $\tint{T}^k$ we get
  \begin{equation*}
      \sem{\lambda x.M}^k_{\nu_k}(\tint{S\cup T}^k)\geq \tint{S\cup T}^k.
  \end{equation*}
  Now we use Lemma~\ref{cor:fixpoints} which tells us that
  \begin{equation*}
    \sem{Y x.M}^k_{\nu_k} = \bigvee
  \set{d \mid \sem{\lambda x.M}^k(d) \geq d\text{ and }  d\down = \sem{Y
      x.M}^{k-1}_{\nu_{k-1}}}\ .
  \end{equation*}
  This gives us immediately the desired $\sem{Y
    x.M}^k_{\nu_k}\geq\tint{S\cup T}^k$. 
\end{proof}

\begin{lem}
  \label{thm:completeness}
  Given a type $S\subseteq \Types^k$ , if $\sem{M}^k_{\sem{\G}^k}\geq \tint{S}^k$
  then $\G\vdash M\geq S$.
\end{lem}
\begin{proof}
  This theorem is proved by induction on the pairs $(M,k)$ ordered
  component-wise.  Suppose that the statement is true for $M$, we are
  going to show that it is true for $Y x.M$, the other cases are
  straightforward.

  The first observation is that, if $T\to S$ is such that $\sem{\lambda x
    .M}^k_{\sem{\G}^k}\geq \tint{T\to S}^k$, then $\G\vdash \lambda x.M\geq
  T\to S$ is derivable. Indeed, since, letting $\nu = \sem{\G,x\geq
      T}^k$, if $\sem{M}^k_\nu\geq \tint{S}^k$ holds then, $\G,x\geq
    T\vdash M\geq S$ is derivable by induction hypothesis. So
    $\G\vdash \lambda x. M\geq T\to S$ is derivable.

    There are now two cases depending on the parity of $k$.  First let
    us assume that $k$ is even. Suppose $\sem{Y x.M}^k_{\sem{\G}^k} =
    \tint{S\cup T}^k$ where $S\incl\types^k$ and $T\incl\Types^{k-1}$.
    Lemma~\ref{lem:sem_representations_with_types} guaranties the
    existence of such $S$ and $T$ as every element of $\Dd^k$ is
    expressible by a set of types.  We have $\sem{\lambda
      x.M}^k_{\sem{\G}^k}\geq\tint{S\cup T}^k\step^k\tint{S\cup
      T}^k$. By the above we get that $\G\vdash \lambda x. M\geq (S\cup
    T)\to(S\cup T)$ is derivable and thus $\G\vdash \lambda x. M\geq (S\cup
    T)\to S$ is derivable as well. We also have $\sem{Y x.M}^{k-1}\geq
    \tint{T}^{k-1}$ which gives that $\G\vdash Y x.M\geq T$ is
    derivable. This allows us to derive $\G\vdash Y x.M\geq S\cup
    T$. Using the subsumption rule and the fact that the subsumption
    reflects the order in the model
    (Lemma~\ref{lem:ordering_correct_complete}),
    every other judgment $\G\vdash
    Y x.M\geq U$ where $\tint{U}^k\leq \sem{Y x.M}^k_{\sem{\G}^k}$ is
    derivable.

  Now consider the case where $k$ is odd. Suppose  $\sem{Y x.M}^k_{\sem{\G}^k} =
  \tint{S\cup T}^k$ with $T\incl \Types^{k-1}$ and $S\incl\types^k$.
  By induction hypothesis on $k$, we have that
  $\G\vdash M\geq T$ is derivable. Take $d=\sem{\lambda
    x. M}_{\sem{\G}_k}^k$. Lemma~\ref{lem:sem_representations_with_types}
  guarantees us a set of types $U\incl \Types^k$ such that
  $\tint{U}^k=d$. By the observation we have made above,
  there is a derivation of $\G\vdash \lambda x.M\geq
  U$. Then iteratively using the rule $Y\ odd$ we compute the
  least fixpoint by letting $U^0(T) = T$ and $U^{n+1}(T) = U(U^n(T))$.
  As in the case above, we can now conclude that for every
  $V\subseteq \Types^k$, if
  $\tint{V}^k\leq \sem{Y x.M}^k_{\sem{\G}^k}$, then $\G\vdash
    Y x.M\geq U$ is derivable.
\end{proof}

As we have seen, the applicative structure $\Dd^k_A$ is a lattice,
therefore each construction can be dualized: in Abramsky's
methodology, this consists in considering $\wedge$-prime elements of
the models, meets and co-step functions instead of $\vee$-primes,
joins and step functions. It is worth noticing that dualizing at the
level of the model amounts to dualizing the automaton.
So, in particular, we can
define a system so that $BT(M)$ is not accepted by $\Aa$ from state
$q$ iff $\G\vdash M \ngeq q$ is derivable.  While the first typing system
establishes positive facts about the semantics, the second one
 refutes them.  For this, we use the same syntax
to denote types, but we give types a different semantics that is dual
to the first semantics we have used. The notation, $\geq$ and $\ngeq$,
we have used for 
the two type systems is motivated by this duality.
\begin{align*}
  \dint{q}^{k} =&\Qlk - \set{q}\ ,\\
  %\sem{q}^-_k&= \set{q'\in Q : \rho(q')\ngeq k \land q'\neq q}\\
  % \sem{S}&= \bigvee \set{\sem{f}: f\in S}\\
  %\sem{S}^-_k&= \bigwedge\set{\sem{f}^-_k: f\in S}\\
  \dint{S \to f}^{k}=& \left(\bigwedge\set{\dint{g}^{k}: g\in
      S}\right)\costep^k \dint{f}^{k}\ .\\
  %\sem{S\to_l f}^-_k&= \sem{S}^-_l \costep \sem{f}^-_k
\end{align*}
% Similarly to the definition of $\tint{\cdot}^k$, we write $\dint{S}^k$
% for $\bigwedge\set{\dint{s}^k: s\in S}$ and we also have that
% $\dint{T\to S}^k = \dint{T}^k\costep^k\dint{S}^k$.  Simply by
% dualizing the proof of the corresponding lemmas for $\tint{\cdot}^k$,
% we can establish the following results:
% \begin{lem}
%   \label{lem:incr_dint}
%   For every type $A$, if $S\incl\Types_A$ and $k\ngeq m$ we have: have
%   that $\dint{S}^k = \dint{S\cap \Types^k_A}$, $\dint{S\cap
%     \Types^k_A}^{k+1} = (\dint{S}^k)\upsup$ and $\dint{S}^k =
%   (\dint{S}^{k+1})\down$.
% \end{lem}

% \begin{lem}
%   \label{lem:sem_representations_with_dual_types}
%   For every $k$ every $A$ and every $f$ in $\Dd^k_{A}$, there is $S$
%   in $\Types^k_{A}$ so that $\dint{S}^{k} = f$.
% \end{lem}
% The subsumption relation for types is defined similarly:
% \begin{center}

% \end{center}

% \begin{thm}
%   \label{thm:ordering_correct_complete}
%   For each $k$, $A$, $S$ and $T$ in $\Types^k_A$, we have that
%   $\dint{S}^{k}\geq\dint{T}^k$ iff $S\tgeq_A T$.
% \end{thm}
% We now define $S(T)$ to be $\set{s : U\to s\in S\land U\tgeq T}$. We
% then have:
% \begin{lem}
%   \label{lem:dint_and_application_commute}
%   For every $k$, $A$ and $B$, if $S\subseteq \Types_{A\to B}$ and
%   $T\subseteq \Types A$, then $\dint{S(T)}^k =
%   \dint{S}^k(\dint{T}^k)$.
% \end{lem}

The dual type system is presented in
Figure~\ref{fig:dual_type_system}. The notation is as before but we
use $\ngeq$ instead of $\geq$.  Similarly to the definition of
$\tint{\cdot}^k$, we write $\dint{S}^k$ for $\bigwedge\set{\dint{s}^k:
  s\in S}$ and we have that $\dint{T\to S}^k =
\dint{T}^k\costep^k\dint{S}^k$. We also need to redefine $S(T)$ to be
$\set{s : U\to s\in S\land U\tgeq T}$. % With those notations, the rules
% for application, abstraction, and variable do not change and are not
% presented in the Figure~\ref{fig:type_system}.
By duality, from
Theorem~\ref{thm:types_correctness_completeness} we obtain:
\begin{thm}
  \label{thm:dual_type_system_correct_and_complete}
  For $S\incl \Types^k$:\quad $\G\vdash M\ngeq S$ is
  derivable iff
  $\sem{M}^k_{\sem{\G}^k} \leq \dint{S}^k$.
\end{thm}

Together
Theorems~\ref{thm:types_correctness_completeness}
and~\ref{thm:dual_type_system_correct_and_complete} give a
characterization by typing of $\sem{M}=L(\Aa)$, that is the set of states from
which our fixed automaton $\Aa$ accepts $BT(M)$.

\begin{cor}
  \label{coro:value_characterization}
  For a closed term $M$ of type $o$:
  \begin{equation*}
    \text{$\sem{M} = \sem{S}$\quad iff\quad both\quad
  $\vdash
  M\geq S$ and\quad  $\vdash M\ngeq (Q-S)$.}
  \end{equation*}
\end{cor}

% \begin{figure*}
%   \centering
%    \begin{prooftree}
%     S\subseteq T\subseteq Q%
%     \justifies%
%     S \tgeq_0 T
%   \end{prooftree}
%   \qquad
%   \begin{prooftree}
%     \forall s \in S, \exists t\in T,
%     s\tgeq_A t%
%     \justifies%
%     S\tgeq_A T
%   \end{prooftree}
%   \qquad
%   \begin{prooftree}
%     T\tgeq_A S\quad s\tgeq_B t%
%     \justifies%
%     S\to s\tgeq_{A\to B} T\to t%
%   \end{prooftree}

%   \medskip

% %   \begin{prooftree}
% %     \justifies%
% %     \G, x \ngeq S \vdash x \ngeq S
% %   \end{prooftree}
% % \quad
% % \begin{prooftree}
% %   \G\vdash M \ngeq S%
% %   \quad
% %   \G\vdash M \ngeq T%
% %   \justifies%
% %   \G\vdash M \ngeq S\cup T%
% % \end{prooftree}
% % \quad
% % \begin{prooftree}
% %   \G\vdash M \ngeq S%
% %   \quad%
% %   T \tgeq  S%
% %   \justifies
% %   \G\vdash M \ngeq T%
% % \end{prooftree}


% % \bigskip

% \begin{prooftree}
% \ %
%   \justifies%
%   \G \vdash c \geq \set{q: \delta_o(q,c)\text{ does not hold}}
% \end{prooftree}
% \quad
% \begin{prooftree}
%   \forall (S_1,S_2)\in\delta(a,q), (T_1\cap S_1)\cup (T_2\cap S_2)\neq \es%
%   \justifies%
%   \G \vdash a \ngeq T_1 \to T_2 \to q%
% \end{prooftree}

% \medskip

% % \begin{prooftree}
% %   \G \vdash M \ngeq S %
% %   \quad%
% %   \G \vdash N \ngeq T
% %   \justifies%
% %   \G\vdash MN \ngeq S(T)%
% % \end{prooftree}
% % \quad
% % \begin{prooftree}
% %   S\in\Types^{k},\, T\subseteq \types^k%
% %   \quad%
% %   \G, x\ngeq S \vdash M\ngeq T%
% %   \justifies%
% %   \G \vdash  \lambda x. M \ngeq S \to T%
% % \end{prooftree}


% % \bigskip

% \begin{prooftree}
%   S \subseteq \types^{2k+1}_{A},\quad%
%   T\in \Types^{2k}_{A},\quad%
%   \G\vdash \lambda x.M\ngeq (S\cup T) \to S%
%   \quad%
%   \G\vdash Y x.M\ngeq T%
%   \justifies%
%   \G \vdash Y x.M\ngeq S\cup T%
%   \using Y\,\mathit{odd}%
% \end{prooftree}


% \medskip

% \begin{prooftree}
%   \G \vdash (\lambda x. M)\ngeq S%
%   \quad%
%   \G\vdash (Y x .M) \ngeq T%
%   \justifies%
%   \G \vdash Y x.M \ngeq S(T)%
%   \using Y\,\mathit{even}%
% \end{prooftree}

% \caption{Dual type system}\label{fig:dual_type_system}

% \end{figure*}



% \subsection{Some leftover proofs}

% \begin{lem}
%   For every type $A$, $S\incl \Types_A$ and $k\leq m$ we have
%   $\tint{S}^k=\tint{S\cap \Types^k_A}^k$.
% \end{lem}
% \begin{proof}
%   Since $\tint{S}^l = \Lor\set{\tint{t}^l : t\in S}$ it is sufficient
%   to show that $\tint{t}^k=\bot^k_A$ for $t\not\in\Types^k_A$. We do it by
%   induction on the type $A$.

%   Suppose that $t\in\types^l_A$ for $l>k$.
%   For type $o$ it follows directly from the definition that
%   $\tint{t}^k=\es$. For $A$ of the form $B\to C$ we know that $t$ is
%   of the form $T\to s$ with $T\incl \Types^k_B$ and $s\in\types^l_C$.
%   By induction assumption $\tint{s}^k=\bot^k_C$. We get $\tint{T\to
%     s}^k=\tint{T}^k\step^k\tint{s}^k=\tint{T}^k\step^k\bot_C=\bot^k_{B\to
%     C}$.\qed
% \end{proof}

% \begin{lem}%\label{lemma:type-up}
%   For every $k< m$ and $A$, if $S\subseteq \Types_A$, then
%   $\tint{S\cap \Types^k_A}^{k+1}=(\tint{S}^k)\upinf$.
% \end{lem}
% \begin{proof}
%   We prove the result only for elements of $\types^k_A$ as the more
%   general one is a direct consequence of that particular case.
%   The proof is by induction on $A$. The base case is obvious. For $A$
%   of the form $B\to C$ we have $\tint{T\to s}^{k+1}$ is by definition
%   $\tint{T}^{k+1}\step^{k+1}\tint{s}^{k+1}$ which by induction
%   hypothesis is $(\tint{T}^k)\upinf\step^{k+1}(\tint{s}^k)\upinf$.
%   We will be done if we show that for every $f\in \Dd^k_B$ and
%   $g\in\Dd^k_C$:
%   \begin{equation*}
%     f\upinf\step^{k+1}g\upinf=(f\step^k g)\upinf\ .
%   \end{equation*}
%   Given $e$ in $\Dd^{k+1}_{B}$,
%   by Corollary~\ref{cor:up-down}, we have $(f\step^{k}
%   g)\upinf(e)$ is equal to $((f\step^k g)(e\down))\upinf$, and
%   therefore:
%   \begin{equation*}
%   (f\step^{k}  g)\upinf(e) =
%   \begin{cases}
%       g\upinf & \text{ if } f\leq e\down, \\
%       \bot^{k+1}_C&  \text{ otherwise}.
%   \end{cases}
%   \end{equation*}
%   Since $f\leq e\down$ iff $ f\upinf\leq e$, by
%   Corollary~\ref{coro:galois_connections}, this  proves the desired
%   equality.
%   \qed
% \end{proof}

% \begin{app_lemma}{\ref{lem:sem_representations_with_types}}
%   For every $k\leq m$ and  every type $A$. For  every $f$ in $\Dd^k_{A}$
%   there is $S\incl\Types^k_{A}$ so that $\tint{S}^{k} = f$, and there
%   is $S'\incl \types^k_A$ so that $\tint{S'}^{k} = \bar f$.
% \end{app_lemma}
% \begin{proof}
%   We proceed by induction on $k$.

%   The case where $k=0$ has been proved in~\cite{SalWalTLCA}.

%   For the case $k >0$, as we have seen with
%   Lemma~\ref{lem:Nn_k_decomposition}, that $f = (f\down)\upinf \vee
%   \overline{f}$. From the induction hypothesis there is $S_1\incl
%   \Types^{k-1}_A$ such that $\tint{S_1}^{k-1}=f\down$. By
%   Lemma~\ref{lemma:type-up} we get $\tint{S_1}^k=(f\down)\upinf$.

%   It remains to describe $\overline{f}$ with types from $\types^k_{B\to
%     C}$. Take $d\in\Dd^k_B$ and recall that $\bar f
%   (d)=\bar{f(d)}$. By induction hypothesis we have $S_d\incl
%   \Types^k_B$ and $S_{\bar{f(d)}}\incl \types^k_{C}$ such that
%   $\tint{S_d}^k=d$ and $\tint{S_{\bar{f(d)}}}^k=f(d)$. So the set of
%   types $S_d\to S_{\overline{f(d)}}$ is included in $\types^k_{B\to C}$ and
%   $\tint{S_d\to S_{\overline{f(d)}}}=d\step^k\bar f(d)$. It remains to take
%   $S_2=\bigcup\set{S_d | d\in \Dd^k_B}$. We can conclude that $S_2\incl
%   \types^k_A$ and $\tint{S_2}^k=\bar f$. Therefore $\tint{S_1\cup
%     S_2}^k=f$.
%   \qed
% \end{proof}

% % \begin{app_theorem}{\ref{thm:ordering_correct_complete}}
% %   For each $k$, $A$, $S$ and $T$ in $\Types^k_A$, we have that
% %   $\tint{S}^{k}\leq\tint{T}^k$ iff $S\tleq_A T$.
% % \end{app_theorem}
% % \begin{proof}
% %   This Theorem is a consequence of the fact that for each $k$, $\Dd_k$
% %   can be embedded in the monotone model generated by $\Pp(\Qlk)$ and
% %   that according to~\cite{salvati12:logical_relation}, the ordering on
% %   intersection types simulate the one in monotone models.\qed
% % \end{proof}

% The main Theorem~\ref{thm:types_correctness_completeness} is proved by
% two lemmas.


% \begin{lem}
%   %\label{lemma:types_correctness}
%   If $\Gamma\vdash M\geq S$ is derivable, then for every $k\leq m$:
%   $\sem{M}^k_{\sem{\G}^k}\geq \tint{S}^k$.
% \end{lem}

% \begin{proof}
%   This proof is done by a simple induction on the structure of the
%   derivation of $\G\vdash M\geq S$.  For most of the rules, the
%   conclusion follows immediately from the induction hypothesis (using
%   Lemmas~\ref{thm:ordering_correct_complete}
%   and~\ref{lem:type_application_is_sem_application}). We shall only
%   treat here the case of the rules $Y\ \mathit{odd}$ and $Y\
%   \mathit{even}$.

%   In the case of $Y\ \mathit{odd}$, when we derive $\G\vdash Y x.M\geq
%   S(T)$ from $\G\vdash \lambda x.M\geq S$ and $\G\vdash Y x.M\geq T$ with
%   $S, T\in \Types^{2l+1}_A$, the induction hypothesis gives that for
%   every $k$, $\sem{\lambda x. M}^k_{\sem{\G}^k}\geq \tint{S}^k$
%   and $\sem{Y x. M}^k_{\sem{\G}^k}\geq \tint{T}^k$.
%   Therefore $\sem{Yx.M}^k_{\sem{\G}^k} = \sem{(\lambda x.M)(Y
%     x.M)}^k_{\sem{\G}^k} \geq \tint{S}^k(\tint{T}^k) = \tint{S(T)}^k$, using
%   Lemma~\ref{lem:type_application_is_sem_application}.

%   In the case of $Y\ \mathit{even}$ we consider the case $k=2l$.
%   Let $\nu_{k-1}$ stand for $\sem{\G}^{k-1}$ and $\nu_{k}$ for
%   $\sem{\G}^{k}$.

%   By induction hypothesis we have $\sem{Y x.M}^{k-1}_{\nu_{k-1}}\geq
%   \tint{T}^{k-1}$. Since Lemma~\ref{cor:L-on-terms} implies $(\sem{Y
%     x.M}^{k-1}_{\nu_{k-1}},\sem{Y x.M}^{k}_{\nu_{k}})\in \lambdal^k$, we have
%   $\sem{Y x.M}^{k}_{\nu_{k}}\geq (\tint{T}^{k-1})\upinf$ by
%   Lemma~\ref{lem:galloi_connections}. By Lemma~\ref{lemma:type-up} we
%   know $(\tint{T}^{k-1})\upinf=\tint{T}^k$. In consequence we have
%   \begin{equation*}
%       \sem{\lambda x.M}^k_{\nu_k}(\tint{T}^k)\geq \tint{T}^k.
%   \end{equation*}
%   Also by induction hypothesis we have $\sem{\lambda x. M}^k_{\nu_k}\geq
%   \tint{(S\cup T)\to S}^k$. This means $\sem{\lambda
%     x.M}^k_{\nu_k}(\tint{S\cup T}^k)\geq \tint{S}^k$. Put together
%   with what we have concluded about $\tint{T}^k$ we get
%   \begin{equation*}
%       \sem{\lambda x.M}^k_{\nu_k}(\tint{S\cup T}^k)\geq \tint{S\cup T}^k.
%   \end{equation*}
%   Now we use Lemma~\ref{cor:fixpoints} telling us that
%   \begin{equation*}
%     \sem{Y x.M}^k_{\nu_k} = \bigvee
%   \set{d \mid \sem{\lambda x.M}^k(d) \geq d\text{ and }  d\down = \sem{Y
%       x.M}^{k-1}_{\nu_{2k-1}}}\ .
%   \end{equation*}
%   This gives us immediately the desired $\sem{Y
%     x.M}^k_{\nu_k}\geq\tint{S\cup T}^k$. \qed
% \end{proof}

% \begin{lem}
%   %\label{thm:completeness}
%   Given a type $S\subseteq \Types^k$ , if $\sem{M}^k_{\sem{\G}^k}\geq \tint{S}^k$
%   then $\G\vdash M\geq S$.
% \end{lem}
% \begin{proof}
%   This theorem is proved by induction on the pairs $(M,k)$ ordered
%   component-wise.  Suppose that the statement is true for $M$, we are
%   going to show that it is true for $Y x.M$, the other cases are
%   straightforward.

%   The first observation is that, if $T\to S$ is such that $\sem{\lambda x
%     .M}^k_{\sem{\G}^k}\geq \tint{T\to S}^k$, then $\G\vdash \lambda x.M\geq
%   T\to S$ is derivable. Indeed, since, letting $\nu = \sem{\G,x\geq
%       T}^k)$, if $\sem{M}^k_\nu\geq \tint{S}^k$ holds then, $\G,x\geq
%     T\vdash M\geq S$ is derivable by induction hypothesis. So
%     $\G\vdash \lambda x. M\geq T\to S$ is derivable.

%     There are now two cases depending on the parity of $k$.  First let
%     us assume that $k$ is even. Suppose $\sem{Y x.M}^k_{\sem{\G}^k} =
%     \tint{S\cup T}^k$ where $S\incl\types^k$ and
%     $T\incl\Types^{k-1}$.
%     Lemma~\ref{lem:sem_representations_with_types} guaranties the
%     existence of such $S$ and $T$ as every element of
%     $\Dd^k$ is expressible by a set of types.  We have $\sem{\lambda
%       x.M}^k_{\sem{\G}^k}\geq\tint{S\cup T}^k\step^k\tint{S\cup
%       T}^k$. By the above we get that $\G\vdash \lambda
%     x. M\geq (S\cup T)\to(S\cup T)$ is derivable and thus $\G\vdash \lambda
%     x. M\geq (S\cup T)\to S$ is also derivable. We also have $\sem{Y
%       x.M}^{k-1}\geq \tint{T}^{k-1}$ which gives that $\G\vdash Y
%     x.M\geq T$ is derivable. This allows us to derive $\G\vdash Y
%     x.M\geq S\cup T$. Using the subsumption rule and
%     Lemma~\ref{thm:ordering_correct_complete}  every
%     other valid judgment $\G\vdash Y x.M\geq U$ is derivable.

%   Now consider the case where $k$ is odd. Suppose  $\sem{Y x.M}^k_{\sem{\G}^k} =
%   \tint{S\cup T}_k$ with $T\incl \Types^{k-1}$ and $S\incl\types^k$.
%   By induction hypothesis on $k$, we have that
%   $\G\vdash M\geq T$ is derivable. Take $d=\sem{\lambda
%     x. M}_{\sem{\G}_k}^k$. Lemma~\ref{lem:sem_representations_with_types}
%   guarantees us a set of types $U\incl \Types^k$ such that
%   $\tint{U}^k=d$. By the observation we have made above,
%   there is a derivation of $\G\vdash \lambda x.M\geq
%   U$. Then iteratively using the rule $Y\ odd$ we compute the
%   least fixpoint by letting $U^0(T) = T$ and $U^{n+1}(T) = U(U^n(T))$.
% \qed
% \end{proof}

% Concerning the dual system, duality on lattices makes it possible to
% derive directly its properties from the previous system. Nevertheless,
% for the sake of completeness, we included the main properties of the
% dual system here (including a complete version of its derivation
% system given Figure~\ref{fig:complete_dual_type_system}).

% Similarly to the definition of $\tint{\cdot}^k$, we write $\dint{S}^k$
% for $\bigwedge\set{\dint{s}^k: s\in S}$ and we also have that
% $\dint{T\to S}^k = \dint{T}^k\costep^k\dint{S}^k$.  Simply by
% dualizing the proof of the corresponding lemmas for $\tint{\cdot}^k$,
% we can establish the following results:
% \begin{lem}
%   %\label{lem:incr_dint}
%   For every type $A$, if $S\incl\Types_A$ and $k < m$ we have: have
%   that $\dint{S}^k = \dint{S\cap \Types^k_A}$, $\dint{S\cap
%     \Types^k_A}^{k+1} = (\dint{S}^k)\upsup$ and $\dint{S}^k =
%   (\dint{S}^{k+1})\down$.
% \end{lem}

% \begin{lem}
%   %\label{lem:sem_representations_with_dual_types}
%   For every $k$, every $A$, and every $f$ in $\Dd^k_{A}$, there is $S$
%   in $\Types^k_{A}$ so that $\dint{S}^{k} = f$.
% \end{lem}


% \begin{lem}
%   %\label{thm:ordering_correct_complete}
%   For each $k$, $A$, $S$ and $T$ in $\Types^k_A$, we have that
%   $\dint{S}^{k}\geq\dint{T}^k$ iff $S\tgeq_A T$.
% \end{lem}
% We now define $S(T)$ to be $\set{s : U\to s\in S\land U\tgeq T}$. We
% then have:
% \begin{lem}
%   %\label{lem:dint_and_application_commute}
%   For every $k$, $A$ and $B$, if $S\subseteq \Types_{A\to B}$ and
%   $T\subseteq \Types A$, then $\dint{S(T)}^k =
%   \dint{S}^k(\dint{T}^k)$.
% \end{lem}




% \begin{center}
%   \begin{prooftree}
%     f\in S%
%     \justifies%
%     \G,x\geq S \vm{k} x\geq f%
%   \end{prooftree}
%   \quad%
%   \begin{prooftree}
%     \rho(q)\ngeq k\quad%
%     \forall (q_1,q_2)\in\delta(a,q),\, q_1\in S_1\lor q_2\in S_2%
%     \justifies%
%     \G \vm{k} a \geq S_1 \to S_2 \to q%
%   \end{prooftree}

%   \bigskip

%   \begin{prooftree}
%     \G \vm{k} M\geq S\to f%
%     \forall g\in S,\, \G\vm{k}N\geq g%
%     \justifies%
%     \G\vm{k} M\geq f%
%   \end{prooftree}

%   \bigskip

%   \begin{prooftree}
%     \G,x\geq S\vm{k} M\geq f%
%     \justifies%
%     \G \vm{k} \lambda x.M \geq S \to f%
%   \end{prooftree}

% \end{center}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "m"
%%% End:



%  LocalWords:  Abramsky's representable BT Yx subsumption fixpoint
%  LocalWords:  iteratively applicative dualized dualizing

